Semantic Segmentation in Satellite Hyperspectral Imagery by Deep Learning

Satellites are increasingly adopting on-board AI to optimize operations and increase autonomy through in-orbit inference. The use of Deep Learning (DL) models for segmentation in hyperspectral imagery offers advantages for remote sensing applications. In this work, we train and test 20 models for multi-class segmentation in hyperspectral imagery, selected for their potential in future space deployment. These models include 1D and 2D Convolutional Neural Networks (CNNs) and the latest vision transformers (ViTs). We propose a lightweight 1D-CNN model, 1D-Justo-LiuNet, which outperforms state-of-the-art models in the hypespectral domain. 1D-Justo-LiuNet exceeds the performance of 2D-CNN UNets and outperforms Apple's lightweight vision transformers designed for mobile inference. 1D-Justo-LiuNet achieves the highest accuracy (0.93) with the smallest model size (4,563 parameters) among all tested models, while maintaining fast inference. Unlike 2D-CNNs and ViTs, which encode both spectral and spatial information, 1D-Justo-LiuNet focuses solely on the rich spectral features in hyperspectral data, benefitting from the high-dimensional feature space. Our findings are validated across various satellite datasets, with the HYPSO-1 mission serving as the primary case study for sea, land, and cloud segmentation. We further confirm our conclusions through generalization tests on other hyperspectral missions, such as NASA's EO-1. Based on its superior performance and compact size, we conclude that 1D-Justo-LiuNet is highly suitable for in-orbit deployment, providing an effective solution for optimizing and automating satellite operations at edge.

==> APPENDICES_FOR_EXTENDED_THESIS.tex <==





\clearpage
\appendix




\section{NOT PART OF THIS PAPER Extended Methodology + State of the art review for the PhD thesis}
\jon{This note is written on 14th October 2023. I have now written the results and the methodology needs to be further compressed since as Radu mentions it has much verbrose including many basic details of Machine Learning and Deep Learning Models. So, what I am doing is to move the methodology as it is now to this appendix section and I will compress and modify/restructure/rewrite the methodology. This previous extended methodology can be used to provide further lower-level and basic details for the extended version of the thesis. NOTE: The section is commented out to avoid messing with the label commands with the rest of the text}

% We present an image ranking system that we have conceptualized, developed, and validated employing real HSI satellite data from the HYPSO-1 mission, as described in the following sections. At the time of writing, the system described next is validated on the ground; however, it is intended for future on-board deployment for inference at the edge on board HYPSO-1. The system is specifically engineered to prioritize HS satellite images for on board post processing, storage and transmission to the ground based on the levels of water, land, and cloud coverage detected in the acquired HS images. Our proposed ranking system will facilitate, during deployment, the option to either discard or apply additional compression to non-essential HSI data at the satellite's edge. Our ranking system already establishes, as per now, a priority queue for HS images, guaranteeing that during deployment those images with higher priority will be post processed and transmitted to the ground first. To build the core of our ranking mechanism, we investigate various ML and DLNN algorithms, assessing their performance \textcolor{blue}{and inference times}. We employ ``The HYPSO-1 Sea-Land-Cloud-Labeled Dataset'', an open dataset introduced in our previous article \cite{justo2023open}, as a use case to demonstrate our ranking system's effectiveness.



% \subsection{An Open Hyperspectral Dataset with Sea-Land-Cloud Ground-Truth from the HYPSO-1 Satellite}

% \radu{There is no need to make such a detailed description of the dataset. One paragraph presenting general statistics (number of images, number of examples, training / test splits) about the dataset should be enough.}

% For our use case scenario, we base our work on the ``The HYPSO-1 Sea-Land-Cloud-Labeled Dataset'' which can be accessed and downloaded freely to facilitate research dissemination from \url{https://ntnu-smallsat-lab.github.io/hypso1_sea_land_clouds_dataset} \cite{justo2023open}. Our dataset, with 200 HS images with spatial resolution of 956 x 684, encompasses approximately 131 million spectral signatures. Each signature contains 120 colors acquired at a spectral resolution of 5 nm from approximately 400 to 800 nm across the visible and part of the Near-Infrared (NIR) spectra. The images in the dataset, collected across all continents, were acquired by the HYPSO-1 satellite mainly during the period from June to December 2022. For constructing the dataset, we prioritized the inclusion of images from coastal and marine environments while ensuring diversity by incorporating scenes of forests, arid landscapes, urban areas, as well as cloud-dominated and overexposed scenarios. The dataset comprises both unprocessed raw and L1b calibrated radiance data serving the dual purpose of extracting insights related to physical radiance units while facilitating comparisons of the radiance data with other satellites. Moreover, in response to the issue of scarce labeled HS imagery, the dataset offers 38 varied images with pixel-level labels, encompassing approximately 25 million labeled spectral signatures across three distinct categories: ``sea'', ``land'', and ``clouds''. The sea category pertains to large saltwater and freshwater bodies, land designates various land covers, and clouds includes both cloud formations and overexposed pixels that obstruct the regions of primary interest. The class distribution is as follows: 37.01\% of the signatures correspond to sea, 40.14\% to land, and 22.85\% to clouds/overexposed areas. This results in a class imbalance with land being the predominant class, with approximately 1.20 land signatures per sea pixel and around 3.31 land signatures per cloud pixel, highlighting the dataset's skewed distribution with clouds as the minority class. When employing the dataset to train ML and DLNN models, this class imbalance may be considered to mitigate bias favoring the majority land class while achieving inferior performance for the minority clouds class, and thereby impacting the model's overall performance. At the time of writing, the current format for downlinking unprocessed raw images from the HYPSO-1 satellite to the ground is the Band Interleaved by Pixel (BIP) format (\textit{.bip}), \textcolor{blue}{where channels for each spectroscopic signature are stored sequentially within each raster image}, and \textcolor{blue}{with each sample} encoded as a 16-bit unsigned integer. To enhance usability, in \cite{justo2023open}, we converted the \textcolor{blue}{raster binary} data format from \textit{.bip} to \textit{.mat}, while preserving the 16-bit unsigned integer data type. The file formats, dimensions, and bit-depths for the raw, L1b radiance data and ground-truth labels in the dataset are outlined in Table \ref{Table:data_and_labels_formats}. Furthermore, we aim to provide further clarity on the dataset by recalling that the sensor arrangement on HYPSO-1 results in raw data channels arranged in decreasing wavelength order from NIR to blue, whereas the radiance data channels are reversed and arranged, during the calibration process, in increasing wavelength order from blue to NIR. \textcolor{blue}{\textbf{JUST CROSSCHECK THE FORMATS, DIMENSIONS, BIT DEPTH AND THE THING WITH THE RASTER.}}


% \begin{table}[h] % 
%   \centering 
%     \caption{Summary of data formats, dimensions, and bit-depths for the data and ground-truth labels.\\UInt.: Unsigned Integer, FloP.: Floating Point} 
%   \begin{tabular}{|c|c|c|c|} 
%     \hline  
%      Data/Labels & Format & Dimensions & Bit Depth \\
%     \hline \hline 
%     Raw & \textit{.mat} & 956 x 684 x 120 & 16-bits UInt.\\
%     \hline
%     L1b Radiance & \textit{.npy} & 956 x 684 x 120 & 32-bits FloP.\\
%     \hline
%     Labels & \textit{.npy} & 956 x 684 & 8-bits UInt.\\
%     \hline
%   \end{tabular}
%   \label{Table:data_and_labels_formats} 
% \end{table}

% Since the start of our work in \cite{justo2023open}, we focused on semantic segmentation of HYPSO-1 images, targeting classes that may be relevant to the HYPSO-1 mission. Initially, our labeling consisted of a detailed pixel-level categorization of these images. Beyond the basic sea, land, and cloud categories, we probed further. For instance, the sea category was subdivided to capture various ocean colors like deep ocean's dark blue or from the turquoise to the darker green colors observed often in shallow waters in the continental shelf, intending in this manner to provide a larger number of rich categories, as it occurs in other conventional datasets such as the Indian Pines dataset from AVIRIS including 16 different categories \textcolor{blue}{[cite]}. Land was also further classified into urban regions, vegetation, arid terrains, and ice-covered areas, among others. However, these detailed and complex categorizations faced the challenges described next. For example, detecting turquoise or green tints in coastal ocean water does not provide enough evidence to assert that these colors stem from a HAB of toxic phytoplankton without costly on-site measurements. Instead, these colors could be attributed e.g. to the interplay of diverse water properties and the seabed. Likewise, this ambiguity and uncertainty are also a concern when it comes to land cover classifications due to the absence of in situ measurements to verify the various land cover subtypes in the ground truth. Therefore, in the context of HYPSO-1, we considered that labeling both water and land coverage into non-conclusive, imprecise, and uncertain subcategories without the validation of on-site measurements were not appropriate for constructing a reliable ground-truth dataset for the research community. Consequently, our labeling effort was restarted with the aim of ensuring not only meaningful, but also reliable and precise labels by an annotation process that was scalable to a larger number of HYPSO-1 images. Our new focus centered on three fundamental simple categories: sea, land, and clouds, for which we had increased confidence benefiting from our expertise in the satellite HSI field. We recall that establishing the reliability of the dataset as a foundational basis for training ML and DLNN models is the initial step that must be guaranteed in this process. However, equally important is the development of a plan for feature analysis, training, validating, and testing the model, as we elaborate in the upcoming sections. 



% \subsection{HSI Data Optimization for On Board Inference: Spectral Anomalies by Isolation Forest and Reduction by Principal Component Analysis}
% Prior to training ML and DLNN algorithms, it is commonly recommended to perform an analysis of the data features. This practice is essential because some of the collected features may not be relevant, could be redundant, or might contain noise that is irrelevant to the algorithm's intended task. This importance is heightened in applications using high-dimensional data such as in HSI, where each spatial pixel does not adhere to the conventional three channels of red, green, and blue. Instead, in an HS image, each pixel contains a multitude of narrow spectral channels. For instance, in the case of the HYPSO-1 mission, the imager captures 120 distinct spectral bands for each spatial pixel. Consequently, dimensionality reduction techniques are often employed as part of the data preprocessing aiming to represent the high-dimensional feature space, $\mathbb{R}^{120}$ in the case of HYPSO-1 data, in a lower-dimensional space $\mathbb{R}^{M}$ with $M<N$, where M denotes the number of reduced color features per pixel. Reducing the number of color features holds significant importance across various aspects of DLNNs applied to HSI data. For instance, this reduction has an impact, notably in terms of kernel components within DLNNs, resulting in a decrease in the overall parameter count. To illustrate, in a 2D-CNN-based network, the number of components in the neural kernels in the first 2D convolutional layer equals the number of components in the input data. Hence, as the number of components in the input image decreases, the number of components in the kernels of the first convolutional layer also gets reduced. This reduction contributes, to a certain extent, to the overall reduction in the model's parameter count. This process of model parameter reduction combined with adequate hyper-parameter tuning, commonly referred to as pruning, plays a crucial role in optimizing the on board storage requirements. The advantages of the color feature reduction extend to computational efficiency, as it translates into fewer operations, leading to on board power savings and faster inference. Moreover, beyond the inference phase, the benefits are also evident during the training process. The reduction in kernel components translates into fewer parameters that need to be trained. This effect is particularly crucial when dealing with 2D-CNN based models. In cases where a large number of color features are present, there is a risk of GPU memory overflow issues, where the operating system (OS) may struggle to allocate all the training tensors from the system random access memory (RAM) into the GPU dedicated memory. Therefore, acknowledging the significance of identifying crucial color features in HS images yet considering the existing literature discussed in the previous state-of-the-art review, which highlights that on-board implementation of dimensionality reduction techniques can consume a substantial amount of power within satellite systems, we conduct the analysis presented next. Using the HSI data from the HYPSO-1 mission, we identify the channels that can be temporarily excluded for the model inference without the necessity of permanently removing them from on board storage. In our use case, the data tensor is a 4th-order tensor with dimensions: \textit{IMAGES} x \textit{LINES} x \textit{SAMPLES} x \textit{CHANNELS}, where \textit{IMAGES} is 38 HS images, \textit{LINES} represents 956 push-broom frames captured sequentially during the satellite's orbital movement, \textit{SAMPLES} indicates 684 slit samples per frame, and \textit{CHANNELS} corresponds to 120 spectral color attributes, as earlier presented in Table \ref{Table:data_and_labels_formats}. Our investigation is divided into the following two distinct stages.


% First, upon transforming the 4th-order data tensor into a 2nd-order tensor, each spatial pixel is transformed into a row including 120 columns representing the spectral attributes. Subsequently, we calculate the standard deviation for each individual color feature across all pixels, resulting in 120 standard deviations. Following an initial examination of the standard deviation distribution among the channels, we utilize the Isolation Forest (IF) anomaly detection algorithm to apply and train on these channel deviations. This algorithm helps identify potential anomalies by distinguishing them from the regular patterns of spectral deviations. The algorithm identifies unusual outliers by assuming that anomalies require fewer tree partitions than regular data points. In particular, the IF algorithm conducts the assessment by using the path length as a score. If a standard deviation has a shorter path length, it is classified as an anomalous deviation, indicating that it diverges from the rest of the data, which might occur, for instance, when dealing with abnormally large values in standard deviations. However, we emphasize that a large channel deviation value does not necessarily provide a definitive conclusion regarding the utility of the spectral channel. For instance, a large standard deviation could indicate either a substantial presence of noisy samples or, conversely, that the channel data exhibits useful variation in its information. Consequently, these anomalous deviations should be viewed as preliminary indicators of outlier deviations, yet without necessarily identifying the underlying cause for these diverged deviations, which must be determined by the human-level expertise in the field. 


% Second, based on the insights from the prior stage, we exclude the channels that are considered uninformative. We provide a more comprehensive discussion of this exclusion of channels in the results section of the paper. Following the removal of these anomalous channels, we proceed with min-max normalization before applying any dimensionality reduction technique. We undertake this normalization, a standard practice before training numerous ML and DLNN algorithms, to guarantee that the data samples share a consistent range. This step accounts for potential outliers with exceptionally large values, preventing them from disproportionately influencing the sensitivity of dimensionality reduction methods towards the input features. The process of min-max normalization is carried out as follows: 


% \begin{equation}
% DATA_{\text{n}} = \frac{DATA - DATA_{\text{min}}}{DATA_{\text{max}} - DATAS_{\text{min}}},
% \end{equation}

% \noindent $DATA_{\text{n}}$ represents each sample in the dataset after normalization, where each sample falls within the range of [0, 1], $DATA$ denotes each sample in the dataset before normalization, and $DATA_{\text{max}}$ and $DATA_{\text{min}}$ refer to the maximum and minimum sample values observed within the dataset, which is used for training, validation, and testing in subsequent stages. As documented in the literature \cite{bakken2022development}, a wide range of techniques for HS images has been investigated from the Principal Component Analysis (PCA) to the Independent Component Analysis (ICA) \cite{lupu2022stochastic}. These are valuable tools to facilitate the analysis of HSI data. In this second stage, where we employ in particular the PCA algorithm, our goal is not to generate a lower-dimensional image for practical use. Instead, our objective is to utilize this reduction technique solely to identify the color characteristics that seem to capture a greater degree of informative variance in a hypothetical PCA reduction process. Therefore, we train a PCA model to convert the high-dimensional color space into a lower-dimensional space consisting of only one principal component $\mathbb{R}^{1}$. From this reduced image, we determine the three color channels that make the most significant contributions to the principal component. Ultimately, these three color characteristics are the feature attributes, $\mathbb{R}^{3}$, we consider pertinent for posterior model inference, as we elaborate further in the results section.


% We do not intend to perform these dimensionality reduction steps on every HS image due to their significant computational requirements, particularly when executed in space. Nonetheless, this analysis serves as an initial step to identify which color channels can be temporarily omitted for ground-based training and, subsequently, for onboard inference. Finally, HSI is renowned for its classification capabilities, primarily because of its wide range of color channels. Therefore, it is natural for questions to emerge when considering the removal of a significant portion of these channels in the HS images. To this extent, we note that despite removing 97.5\% of the channels (117 channels), the remaining 3 channels \textcolor{blue}{offer a high resolution not found in the standard RGB imaging}. Thus, \textcolor{blue}{utilizing these 3 narrow HS channels offers benefits that extend beyond reducing on board memory demands and power consumption}. Furthermore, our decision to employ 3 channels aligns with current literature for on board AI for object recognition, which predominantly favors this approach over using the entire array of color channels \textcolor{blue}{[cite soa from the previous review]} \textcolor{blue}{(this last paragraph (from finally, ...) may be removed about the three HS channels)}. 





% \subsection{Training/Validation/Testing/Deployment Sets Partitioning}
% After eliminating certain color features as well as normalizing the resulting dataset through min-max normalization, we proceed to partition the data into training, validation, and test subsets at the image level.

% Taking into account the acceptable performance results obtained in our prior work training a 1D Fully Convolutional Neural Network (FCN) for pixel-level segmentation \cite{justo2023open}, we maintain the same data split in this current work. This entails allocating approximately 79\% of the data for training, 8\% for validation, and 13\% for testing. Namely, we use 30 training images, which contain approximately 20 million spectral signatures, making extensive use of the dataset for the training process. For validation, we employ 3 images, amounting to around 2 million signatures. While validation images play a crucial role in iterative hyperparameter model fine-tuning for batch learning in DLNNs, we decide to prioritize the utilization of a slightly larger number of images for testing to evaluate the model's performance on unseen HYPSO-1 data. Therefore, the test set comprises 5 images, containing approximately 3 million signatures. Table \ref{Table:subsets_imbalance} displays the class imbalances for the various subsets. In both the training and test subsets, the majority class is ``land'', while in the validation subset, the majority class results to be in ``sea'' due to the random split. The table offers information on class distribution in terms of percentages and imbalance ratios. The imbalance ratios are presented in the format 1:X, signifying that for each instance of the corresponding non-majority class, there are X instances of the dominating class. To ensure the reproducibility of our research, we offer additional information regarding the particular images employed for training, validation, and testing. We provide image metadata such as geopgrahical location, their corresponding RGB-color composites and ground-truth labels. This information is found in the supplementary Appendix \ref{Appendix: IDs_for_training_validation_and_test_images} \textcolor{blue}{(great if we can mention the location of the scenes for the subtsets)}. 


% Finally, to assess the model's performance beyond 5 images from the test subset, we establish an additional subset referred to as the \textit{deployment subset}. This subset consists of \textcolor{blue}{20} HS images from The HYPSO-1 Sea-Land-Cloud Dataset \cite{justo2023open}. This new subset serves a crucial purpose: it allows us to better evaluate how the model would perform when deployed on board HYPSO-1. In the real-world scenario, the model will encounter new, unseen images. This deployment subset is an extension of the model's testing subset including merely 5 images due to the finite ground-truth data. The deployment subset provides further evaluation, aiming to confirm the model's ability to generalize effectively. However, unlike the test subset, the deployment subset does not have ground-truth labels, and therefore we must rely on e.g. the model's probabilistic confidence when making the predictions for each class. Furthermore, in this case, the combination of visual qualitative assessment aligns with the methodologies employed by fellow researchers in the field, as indicated in the literature \textcolor{blue}{[ref in soa]}. Our accumulated expertise in the HSI field serves as the foundation for this qualitative assessment procedure for the model's further generalisation. 


% \begin{table}[h]
%   \centering
%   \caption{Class imbalance across subsets}
%   \begin{tabular}{|c|c|c|}
%     \hline
%     Subset & Distribution Ratio & Imbalance Ratio \\
%     \hline \hline

    
%     \multirow{3}{*}{Training} & \multirow{3}{*}{\shortstack{Sea: 35.25\% \\ Land: 40.23\% \\ Clouds: 24.52\%}} & \multirow{3}{*}{\shortstack{SEA: 1:1.14 \\ Land: Majority \\ Clouds: 1:1.64}} \\
%     && \\
%     && \\
%     \hline



%     \multirow{3}{*}{Validation} & \multirow{3}{*}{\shortstack{Sea: 51.25\% \\ Land: 28.13\% \\ Clouds: 20.62\%}} & \multirow{3}{*}{\shortstack{Sea: Majority \\ Land: 1:1.82 \\ Clouds: 1:2.49}} \\
%     && \\
%     && \\
%     \hline


%     \multirow{3}{*}{Testing} & \multirow{3}{*}{\shortstack{Sea: 39.01\% \\ Land: 46.85\% \\ Clouds: 14.13\%}} & \multirow{3}{*}{\shortstack{SEA: 1:1.20 \\ Land: Majority \\ Clouds: 1:3.31}} \\
%     && \\
%     && \\
%     \hline

    
%   \end{tabular}
%   \label{Table:subsets_imbalance}
% \end{table}







% \subsection{Spectral and Spatial Contexts in HSI Data: 1D and 2D Data Processing}
% AI models produce predictions for what are widely referred to as data points. Particularly, in the context of our work and with regard to our dataset, since the segmentation models generate a sole prediction for each individual pixel, we refer to each pixel unit as a data point, consisting of multiple 1D color features. The inference process of our models operates in the following two modes: one where it handles one data point at a time, and another where it concurrently processes multiple data points within the same inference process, regardless of whether multiple inference processes are parallelized with e.g. edge computing. When the inference process handles one data point at a time, such as a 1D spectral signature in our context, we refer to the model as a 1D model. Models of this type, such as 1D-CNN-based models, solely consider the spectral characteristics of the pixels to make predictions. On the other hand, when the inference process handles simultaneously multiple neighboring spatial pixels, we refer to these models as 2D models. These models, like 2D-CNN-based models, incorporate a 2D context that encompasses information from both the spectral (color) and spatial (location) domains. In other words, 2D models consider both the color and the arrangement of pixels in their predictions. While 2D models offer advantages by considering neighboring spatial information, which can help compensate for issues in HSI-equipped satellites like inter-band misalignment \textcolor{blue}{[thesis HYPSO ref]}, they come with the downside of increased parameter count and memory requirements and more computations leading to higher power consumption. In contrast, 1D models, which lack spatial context and may be more susceptible to inter-band misalignment, have the benefit of fewer parameters to store in on board memory and \textcolor{blue}{fewer computational operations during inference} \textcolor{blue}{(this last paragraph since where it says: while 2D models offer advantages ... really needs to be revised}.

% \textcolor{blue}{(WARNING: The following paragraph will be changed - all the models are tested using 3 channels and also using most of the channels).} When dealing with 1D models to analyze data points, we utilize nearly all available channels, excluding those that lack significant relevance for multi-class classification. In the context of 1D models, it is practical to retain most color features due to the reduced complexity of these models. This is additionally important for 1D approaches since these models solely consider color context and do not take spatial context into account. In contrast, for 2D models, we exclude most bands, utilizing only three essential color channels following the analysis in the previous section. This omission of color attributes is acceptable for 2D models because they benefit from neighboring spatial pixels to enhance the predictions. An adequate color reduction is critical for 2D models, as it facilitates training on standard industry GPUs, given the inherent complexity of these models. By reducing the number of channels to be fed into 2D models, we also minimize the kernel components and \textcolor{blue}{computational operations} across layers. Concrete color wavelengths included and excluded for 1D and 2D processing are elaborated upon in the results section \textcolor{blue}{(THIS PARAGRAPH IS UNDER WARNING - It is not incorrect, but it will be adjusted and updated)}.


% In 1D processing, the image is transformed from a 3rd-order tensor into a 2nd-order tensor, with the spatial pixels forming rows and their respective spectral features forming columns, resembling the tabular data format commonly used in fields like genetics within bioinformatics \textcolor{blue}{[cite]}. For the remaining images in e.g. the training subset, we also add subsequently the corresponding data points associated with those images. We apply the same procedure for the validation and test subsets. When training the 1D models, we use the term batch samples to refer to the data points where, in this context, each batch sample consists of a 1D spectral signature. The 1D models in the upcoming sections are designed to take inputs formatted as \textit{BATCH SIZE} x \textit{CHANNELS}, with \textit{BATCH SIZE} denoting the number of spectral signatures processed in each mini batch for DLNN training. 


% In 2D processing, it is crucial to optimize both memory usage and computational resources during the inference process while also ensuring that the training can be completed within a reasonable time frame. To achieve this, rather than passing the entire image to the model, we divide it into smaller subimages commonly known as patches or tiles. These patches have reduced spatial dimensions, and each patch is also represented as a 3rd-order tensor, encompassing both the spectral and reduced spatial dimensions. Similarly to what we presented for the 1D case, for the rest of the images in e.g. the training subset, we also append the rest of the patches across the images in the subset. We also apply the same procedure for the validation and test subsets. When training 2D models, each batch sample consists of a 2D patch. In order to guarantee an integer number of patches in both the \textit{lines direction} and the \textit{samples direction}, we modify the data through either cropping or padding, as explained next, and we apply this process to all the mentioned subsets. While we implement cropping and padding, this work focuses primarily on padding. The motivation behind this choice is that cropping leads to the loss of information at the image edges which may be potentially valuable in some cases and that cannot be retrieved back. Therefore, we find it more suitable to add padding to the top, bottom, and side edges to prevent any loss of information. While the padding approach may introduce e.g. some minimal redundant data, the padded borders in the predicted images can be easily removed by cropping the extra lines and samples added during padding. 

% Next, we provide additional details on the cropping and the padding. First, as a result of cropping, the dimensions of lines and samples in the image are adjusted as per the following equations:

% \begin{align}
% \text{LINES'} &= \left\lfloor \frac{\text{LINES}}{\text{PATCH SIZE}} \right\rfloor \times \text{PATCH SIZE}, \text{and} \\
% \text{SAMPLES'} &= \left\lfloor \frac{\text{SAMPLES}}{\text{PATCH SIZE}} \right\rfloor \times \text{PATCH SIZE},
% \end{align}

% \noindent where the values LINES' and SAMPLES' represent the lines and samples of the cropped image, respectively. The expressions \( \left\lfloor \frac{\text{LINES}}{\text{PATCH SIZE}} \right\rfloor \) and \( \left\lfloor \frac{\text{SAMPLES}}{\text{PATCH SIZE}} \right\rfloor \) designate, respectively, the number of patches in the cropped image along the lines and samples directions, with \( \left\lfloor \right\rfloor \) denoting the floor rounding operation. The total number of lines cropped from the image's top and bottom edges combined is given by \( \text{LINES} - \text{LINES'} \) and the number of samples cropped from the image's sides is given by \( \text{SAMPLES} - \text{SAMPLES'} \). When dividing the cropped lines between the top and bottom edges (or similarly, between the left and right sides for samples), we split them evenly. If the number is odd, we crop an additional line (or sample) from the bottom (or right side) of the image. However, for our selected method, padding, the dimensions of lines and samples in the padded image are adjusted as per the equations:

% \begin{align}
% \text{LINES'} &= \left\lceil \frac{\text{LINES}}{\text{PATCH SIZE}} \right\rceil \times \text{PATCH SIZE}, \text{ and} \\
% \text{SAMPLES'} &= \left\lceil \frac{\text{SAMPLES}}{\text{PATCH SIZE}} \right\rceil \times \text{PATCH SIZE},
% \end{align}

% \noindent where LINES' and SAMPLES' denote the lines and samples of the padded image. Using the ceiling function \( \left\lceil \right\rceil \), \( \left\lceil \frac{\text{LINES}}{\text{PATCH SIZE}} \right\rceil \) and \( \left\lceil \frac{\text{SAMPLES}}{\text{PATCH SIZE}} \right\rceil \) indicate the number of patches along the lines and samples. The differences \(\text{LINES'} - \text{LINES} \) and \(\text{SAMPLES'} - \text{SAMPLES} \) represent the total padded lines and samples. Similarly to cropping, we distribute the padding also evenly between top and bottom (or left and right for samples). If uneven, an extra line (or sample) is added to the bottom (or right). For the padding strategy, we consider two approaches to assign values to the padded samples. The first involves incorporating distinctive data into a dedicated padding category for the extended pixels. The second option is to extend the padded pixels to align with the borders of both the data and the annotated images. This results in a visual effect resembling an image with smoothly shifted borders, similar to a moving image. We opt for the second option to avoid introducing an artificial padding category, as it would occur in the first alternative, in order to preserve the consistency of both the images' content and annotations. Additionally, any shift effect at the edges can be partially mitigated by cropping the padded lines and samples along the borders, as previously mentioned. 


% After we pad the data and annotations, we proceed to partition the images into an integer number of patches for the training, validation, and test subsets. To ensure the reproducibility of our data preprocessing pipeline, we provide next the dimensions of both the data and annotations right before and after patching. Namely, before patching, the data is organized as a 4th-order tensor with dimensions \textit{IMAGES} x \textit{LINES} x \textit{SAMPLES} x \textit{CHANNELS}, while the categorical annotations are structured as a 3rd-order tensor with dimensions \textit{IMAGES} x \textit{LINES} x \textit{SAMPLES}. The ground-truth annotations from the HYPSO-1 Sea-Land-Cloud Dataset have values ranging from [0, 2] \cite{justo2023open}, where category 0 represents a sea pixel, category 1 denotes a land pixel, and category 2 signifies a pixel that is either cloudy or overexposed. When we patch the data and annotations, an additional two dimensions are introduced to represent the patch map generated for each image. Consequently, the data and annotations are transformed into 6th-order and 5th-order tensors, respectively. These tensors have the following dimensions. Data: \textit{IMAGES} x \textit{NUMBER OF PATCHES IN LINES DIRECTION} x \textit{NUMBER OF PATCHES IN SAMPLES DIRECTION} x \textit{PATCH SIZE} x \textit{PATCH SIZE} x \textit{CHANNELS}. Categorical annotations: \textit{IMAGES} x \textit{NUMBER OF PATCHES IN LINES DIRECTION} x \textit{NUMBER OF PATCHES IN SAMPLES DIRECTION} x \textit{PATCH SIZE} x \textit{PATCH SIZE}, i.e., the annotated labels have similar dimensions as the data, yet without the \textit{CHANNELS} dimension. When patching the data and annotations, we have explored both overlapping and non-overlapping patching strategies. Overlapping patching offers advantages by introducing redundant data at patch borders, which can enhance analysis in these border regions. However, we have chosen non-overlapping patching to guarantee that each data point is processed only once. This choice enhances computational efficiency during training and eliminates the need to handle data overlaps. The 2D models presented in the following sections are configured to take inputs of the shape \textit{BATCH SIZE} x \textit{PATCH SIZE} x \textit{PATCH SIZE} x \textit{CHANNELS}, with \textit{BATCH SIZE} representing the number of patches processed in each mini batch step in the case of DLNN training. To fit this format, the training, validation, and test data after patching — in 6th-order and 5th-order tensors for data and annotations respectively — need to be further reshaped. After this resize, the data gets the needed dimensions of \textit{BATCH SIZE} x \textit{PATCH SIZE} x \textit{PATCH SIZE} x \textit{CHANNELS}, while the categorical annotations acquire dimensions \textit{BATCH SIZE} x \textit{PATCH SIZE} x \textit{PATCH SIZE}. In both cases, \textit{BATCH SIZE} represents the total number of patches within the subset.




% \subsection{Other Data Preprocessing Considerations: Data Augmentation and Class Balance}
% We have considered incorporating additional data preprocessing steps. Nevertheless, as evidenced in the subsequent results section in this article, the results we have achieved without these preprocessing steps are considered satisfactory for the HYPSO-1 use case, and consequently, we have not found it necessary to implement any of the processing stages mentioned in this concrete section. Certain processing steps, such as data augmentation, are sometimes employed to address issues like insufficient varied training data and hence improve the ability of trained models to generalize better to unseen data. Furthermore, data augmentation may be especially advantageous in certain situations when patching is employed, as patched images expand the range of potential combinations for augmentation operations across the dataset. However, the data augmentation methods we have initially assessed range from basic geometric transformations like rotations and scalings \textcolor{blue}{[geometric transformations in HSI]} to more advanced techniques rooted in Generative AI, such as the use of Generative Adversarial Networks (GANs) (\textcolor{blue}{[cite for GANs in HSI]}, which aim to generate artificial images that closely resemble real data. However, in our specific case, since our work relies on the HYPSO-1 Sea-Land-Clouds-Labeled Dataset \cite{justo2023open}, we do not utilize data augmentation techniques as the results indicate that the dataset sufficiently supports training ML and DLNN models for inference on board HYPSO-1. Beyond data augmentation, we have also contemplated using additionally class oversampling or subsampling to address the dataset imbalance. Nonetheless, we opt against altering the class instances for the same reason as previously mentioned in relation to our performance results. The results unequivocally suggest that, at least at the time of writing, there may not be a strict necessity to modify class instances to attain a more balanced dataset for the preliminary tests of experimental AI on board the HYPSO-1 mission.




% \subsection{Modeling ZZZZZZZ - TO BE FILLED IN}
% \textcolor{blue}{To be filled in with multiple block diagrams for all models + description}
% % Specify how and why the models have been adjusted in this work
% %% NB!! The NB is GaussianNB


% %%%%%% JON: The following calculation for the number of parameters needs confirmation from Lily
% %%% CALCULATION OF NUMBER OF MODEL PARAMETERS IN SGD:
%         % numer_of_model_parameters = len(model_classifier.coef_.ravel()) + NUMBER_OF_CLASSES_DL  # Adding 3 as interpet since there is one intercept per class (3 classes)
% %%% CALCULATION FOR GAUSSIAN NAIVE BAYES:
%     % n_features = 3 # or whatever number of features we have, it could be for instance 112 features
%     % n_classes = len(model_classifier.classes_)
%     % numer_of_model_parameters = 2 * (n_features * n_classes + n_classes)
    
% %%% CALCULATION FOR LINEAR DISCRIMINAT ANALYSIS TRAINED WITH 'SVD': 
%     % n_features = 3 # or whatever number of features we have, it could be for instance 112 features
%     % number_of_params_means = np.prod(model_classifier.means_.shape)  # Number of parameters referring to means
%     % number_of_params_cov = n_features * (n_features + 1) // 2  # Number of parameters referring to the shared covariance matrix (unique ones due to symmetry)
%     % number_of_params_priors = len(model_classifier.priors_) - 1  # Number of parameters referring to priors
%     % numer_of_model_parameters = number_of_params_means + number_of_params_cov + number_of_params_priors


% %%%% CALCULATION FOR THE QUADRATIC DISCRIMINANT ANALYSIS: 
%     % n_features = 3 # or whatever number of features we have, it could be for instance 112 features
%     % n_classes = len(model_classifier.classes_)
    
%     % number_of_params_means = np.prod(model_classifier.means_.shape)  # parameters for means
%     % number_of_params_cov = n_classes * (n_features * (n_features + 1) // 2)  # parameters for covariance matrices
%     % number_of_params_priors = len(model_classifier.priors_) - 1  # parameters for priors
%     % numer_of_model_parameters = number_of_params_means + number_of_params_cov + number_of_params_priors
    




% %%% Specify clearly the input and output dimensions
% %%% Mention that only for ML, but also for DLNN
% %%% No 2D for ML, but only for DLNN (reason: sklearn implementation)
% %% ZZZZ what is the output of the models (for ML and for DLNN: probability) ZZZ
% %%% For results: the number of models we have trained through hyper-parameters (of the ones we are actually giving)


% \subsubsection{Model 1 (ML): Stochastic Gradient Descent}

% \subsubsection{Model 2 (ML): Naive Bayes}

% \subsubsection{Model 3 (ML): Linear Discriminant Analysis}

% \subsubsection{Model 4 (ML): Quadratic Discriminant Analysis}


% \subsubsection{Model 5 (DLNN): Liuetal} % then huetal..., etc

% \begin{figure}[htbp]
%     \centering 
% \includegraphics[width=0.45\textwidth]{Figures/Sample_architecture_from_previous_paper.png} 
%     \caption{\textcolor{blue}{The block diagrams will have this style}}
%     \label{Fig:} 
% \end{figure}




% %%% Specify clearly the input and output dimensions

% \subsubsection{Model 1 (DLNN): Full U-Net} % etc....










% \subsection{A Novel Sea-Land-Clouds Ranking System for Efficient On-Board Edge Data Management}
% We explore deeper into the usability of identifying on board the HYPSO-1 satellite the sea, land, and cloud categories, despite their relative simplicity. We elaborate on how on-board sea-land-cloud segmentation can enhance HYPSO-1's intelligent capabilities, transforming it into a more autonomous satellite. This segmentation allows for improved on board data management, reducing postprocessing, decreasing latency between data acquisition and the decision-making process, all while optimizing the efficient use of the Shannon channel capacity by transmitting only valuable and meaningful data within the restricted downlink, which is a common bottleneck in many satellites like HYPSO-1 operating additionally in limited LOS conditions \cite{Bakken2023}. When constructing the HYPSO-1 Sea-Land-Clouds Labeled dataset in \cite{justo2023open}, as well as during the model training, validation, and testing phases in this work, our primary focus lies in recognizing that our sea-land-clouds segmentation system is designed to serve as the fundamental keystone for the intelligent ranking system we are about to propose. To the best of our knowledge \textcolor{blue}{[all SoA studied]}, our novel ranking system stands as the first approach within the domain of on board space applications specifically tailored for satellites equipped with HSI technology. Unlike the current state-of-the-art systems, which, as of the time of writing, predominantly concentrate solely on clouds, our system distinguishes itself by introducing a unified approach that simultaneously identifies and ranks water and land, beyond clouds, within a priority queue, as explained next. 


% Fig. \ref{Fig:flow_chart_ranking_system} illustrates a flow diagram of our proposed ranking system intended for future deployment on board HYPSO-1. Upon capturing an image, it undergoes processing by a segmentation model that assigns each image pixel to a unique of three distinct categories: sea, land, or clouds/overexposed. Just like monitoring satellite health status through telemetry, we propose saving the segmented sea-land-cloud images in a compact thumbnail format, at least for the initial experimental tests in space. This compact format helps conserve memory storage while preventing overloading the downlink, making it easier for operators to conduct tests and gain insights into the experimental segmentation process. As each pixel in the segmented image is assigned to a specific category, we compute the predicted cloud coverage level using the following equation:


% \begin{equation}
%     \text{Cloud Coverage} = \frac{\text{Cloudy Pixels}}{\text{Total Pixels}}.
% \end{equation}

% Subsequently, the cloud coverage may be compared to a configurable experimental cloud threshold $TH_{cl}$, which may be defined by the ground operators. In the literature, specifically concerning the HyperScout-2 data from the Phi-Sat-1 mission \textcolor{blue}{[ref]}, it is noted that a threshold of 70\% cloud coverage is employed to determine when an image is classified as ``fully cloudy''. If the cloud coverage level exceeds $TH_{cl}$, it indicates an undesirable scenario with an excessive number of cloudy pixels. Consequently, the image can be safely removed from the on board memory, eliminating the necessity for additional postprocessing or downlink. Conversely, when the image does not exhibit a critical cloudy ratio that renders it useless, we proceed with further analysis of the segmented result. In this more favorable scenario, there is a possibility of valuable spectral pixels representing either sea or land. In this scenario, we first determine the primary objective of the satellite's campaign, which helps us prioritize between sea or land data. This is crucial since it enables us to streamline the data, focusing only on the pertinent data, and thereby minimize the processing and downlink of irrelevant information. For instance, if the objective of HYPSO-1's campaign is to monitor the ocean for phenomena such as HABs, other marine events, floating debris, or oil spills, an image showing minimal water content would be considered irrelevant for the campaign's purpose. Indeed, pointing inaccuracies and other satellite operational issues can sometimes result in the imager capturing areas not aligned with the campaign's objective whatsoever. Likewise, if HYPSO-1 is tasked with monitoring terrestrial events, such as fire prevention or tracking wildfires, but the satellite captures an image primarily containing oceanic data, the scene would not be useful to the campaign's purposes. In essence, regardless they are sea or land pixels, their relevance is determined by the campaign's concrete objectives, somewhat similar as with cloud pixels.



% In the event that the campaign focuses on water observation, the predicted sea level, computed similarly to the cloudy coverage level previously shown, is compared to a configurable sea coverage threshold denoted as $TH_{sea}$. This comparison ensures that the image contains a minimum ratio of water pixels. If the predicted sea coverage level falls below the threshold $TH_{sea}$, it indicates an undesirable situation where there are too few water pixels for the mission's focus on observing water systems. Consequently, the image scene is discarded. Conversely, if the sea coverage level exceeds the threshold $TH_{sea}$, it indicates the presence of a sufficient number of sea pixels which are of value for the campaign. In this case, pixels classified as irrelevant (such as cloudy and land pixels) can either be completely discarded or significantly degraded in encoding by reducing them below the data's intrinsic entropy. This process leads to a reduction in the amount of binary data to be handled in subsequent on board postprocessing steps, resulting in power savings for the satellite merely as regards to the postprocessing computations and transmission radio power. Regardless if the irrelevant data is discarded or compressed through the mentioned lossy compression, the image is subsequently queued based on the predicted sea coverage level. This queue determines the downlink priority when the satellite establishes LOS communication with its ground stations, and hence the system, upon deployment, would optimize the downlink usage with the transmission of only relevant data. Fig. \ref{Fig:flow_chart_ranking_system} illustrates that when the campaign is, however, centered around terrestrial land observation, the predicted land coverage level becomes central in assessing whether it falls below or exceeds the predefined threshold $TH_{land}$, much like the methodology depicted in Fig. \ref{Fig:flow_chart_ranking_system} for water-centric campaigns. The distinction lies in considering land pixels as relevant, while categorizing sea and cloudy pixels as irrelevant for the campaign's purpose. 

% \begin{figure*}[ht]
%   \centering
%   \resizebox{1.3\columnwidth}{!}{\includegraphics{Figures/flow_chart_ranking_system.png}}
%   \caption{\textcolor{blue}{Visibility of the figure/do not write post-processing (remove -)}}
%   \label{Fig:flow_chart_ranking_system}
% \end{figure*}




% Considering the ranking system illustrated in Figure \ref{Fig:flow_chart_ranking_system}, we present next the metrics that hold greater significance when assessing the performance of the sea-land-cloud segmentation models on the test subset. These metrics rely on comparisons with ground-truth annotations and are crucial for evaluating the models' suitability for generalization to unseen data. In the context of the presented multi-class classification problem, we approach the evaluation of model performance for each specific class by treating them first as separate binary classification problems as follows. 


% To begin, we establish the definitions for true positive, true negative, false positive, and false negative ratios. We commence by focusing only on the clouds category. In cloud binary classification, a prediction can fall into either the positive or negative category. When a prediction is deemed positive, it signifies that the model identifies a pixel as belonging to the cloud category. Conversely, when a pixel receives a negative prediction, it indicates that it does not correspond to clouds. Instead, it corresponds to either sea or land data. Regardless of whether a prediction is positive or negative, it can also be categorized as either true or false based on the respective ground-truth label. A true prediction indicates that the model correctly predicts the category for the pixel when compared to the ground-truth data. Conversely, a false prediction indicates that the model's prediction is incorrect and does not align with the expected outcome observed in the ground-truth annotation. A false positive for clouds occurs when the alarm is triggered despite the absence of clouds, while a false negative signifies that the alarm fails to trigger when clouds should have been detected. Using these definitions for positive and negative predictions, as well as true and false predictions, we define next four distinct alarm rates. As shown in the following equations, the true alarm rates include the rates of true positives (TPR) (\ref{Equation:TPR}) and true negatives (TNR) (\ref{Equation:TNR}), which determine the correctness of the predictions. The TPR, sometimes referred to as recall or hit rate, quantifies the model's ability to identify ground-truth positive instances for clouds. In contrast, the TNR assesses the model's capacity to correctly identify non-cloudy pixels among all the true non-cloudy samples. Conversely, the false alarm rates encompass the rates of false positives (FPR) (\ref{Equation:FPR}) and false negatives (FNR) (\ref{Equation:FNR}), which evaluate the degree of error in the model's predictions. The FPR, occasionally called the fallout rate, quantifies the ratio of instances where the positive alarm for clouds is triggered, even when it should not have been activated. In contrast, the FNR, also known as the miss rate, represents the ratio of cases in which a positive alarm for clouds should have been triggered but was not. The equations for the ratios are given next: 

% \begin{equation}
%     TPR = \frac{TP}{\text{GT Positives}} = \frac{TP}{TP + FN},
%     \label{Equation:TPR}
% \end{equation}

% \begin{equation}
%     TNR = \frac{TN}{\text{GT Negatives}} = \frac{TN}{TN + FP},
%     \label{Equation:TNR}
% \end{equation}


% \begin{equation}
%     FPR =\frac{FP}{\text{GT Negatives}} = \frac{FP}{FP + TN},
%     \label{Equation:FPR}
% \end{equation}

% \begin{equation}
%     FNR = \frac{FN}{\text{GT Positives}} = \frac{FN}{FN + TP},
%     \label{Equation:FNR}
% \end{equation}, 

% \noindent where GT Negatives denote the ground-truth pixels corresponding to non-cloud targets, i.e., sea and land pixels, while GT Positives represent the ground-truth pixels that depict true clouds. In an ideal scenario, models should exhibit high true alarm ratios while maintaining low false alarm ratios. However, these ratios involve a trade-off, and their relationship does not necessarily follow a linear pattern, as often observed in Receiver Operating Characteristics (ROC) figures where TPR is plotted against FPR revealing that an increase in true positive predictions frequently coincides with a rise in false positive predictions \textcolor{blue}{[cite to ROC often increasing]}. In our ranking system, we prioritize the assessment of the FPR and FNR since these ratios offer direct insights into incorrect positive and negative predictions, as elaborated next. 


% In the context of clouds, the TPR relates to the accurate identification and proper handling, such as discarding or applying lossy compression, of cloudy pixels that are irrelevant. Conversely, the TNR relates to the recognition of data that holds potential value as it does not correspond to clouds. In this scenario, these non-cloudy pixels should not be subjected to discard or lossy compression, considering their informational value. Nevertheless, when dealing with clouds, we explain next why the crucial metric to consider is the FPR. This rate is key since it relates to pixels that have been incorrectly predicted as clouds, even though they are, in reality, sea or land. Essentially, the model misidentifies these pixels as irrelevant clouds, despite they actually correspond to relevant data (sea or land). Consequently, this data is either discarded despite its potential value, resulting in an irreversible loss of valuable net information or, in the best case, applying lossy compression leading to a degradation in the data quality representation. Both data discard and lossy compression are undesirable outcomes stemming from the model's misclassification of data as clouds. Moreover, still in the clouds binary context, the FNR also holds relevance. The FNR signifies that instances where pixels actually correspond to clouds are incorrectly identified as potentially valuable sea or land data. Consequently, in such cases, there is no elimination or lossy compression applied to these superfluous cloudy pixels, even though they are irrelevant. Nonetheless, while the FNR remains an important consideration due to its contribution to the inefficient use of the downlink capacity, where superfluous cloudy data is transmitted without degradation, the FNR is still considerably less critical than the FPR. The FPR is of critical importance since this ratio relates to the irreversible loss of data through discard or subjecting the data to significant degradation by lossy compression. In summary, both FPR and FNR are vital metrics that share a trade-off, where reducing the FPR often leads to an increase in the FNR. However, for the specific context of clouds segmentation in our ranking system, the FPR takes precedence due to its relation with the potential for the model causing irreversible loss of valuable data. In contrast, the FNR primarily relates to optimizing the efficient usage of the downlink posing no risk of data loss. 


% Next, to evaluate the performance of segmentation models for the binary sea class, we begin by considering a scenario where the primary objective is to observe and identify water systems rather than land terrains. When a pixel is a true positive for the sea category, it implies the correct identification of valuable water data for the campaign's objective, affirming that this pixel should be retained without compromising its encoding quality. Conversely, when a pixel is labeled as a true negative for the sea class, it indicates the correct recognition of non-relevant data (such as land or clouds) for the mission's campaign, justifying its potential discard or degradation through lossy compression. However, in the context of a sea-focused campaign and in contrast to our previous conclusion for cloudy scenarios, the FNR becomes of critical concern in this case. The FNR relates to the scenario where a pixel is incorrectly classified as non-relevant sea-related information (land or clouds), consequently misidentifying the pixel as insignificant for the campaign's goals. This misclassification results in either the discard or lossy compression degradation of the pixel containing water information, and hence leading to irreversible loss of valuable data. In contrast to the cloud scenario previously discussed, where FPR is of critical importance, in the context of binary sea classification, the FPR is less critical than FNR, as explained next. In the case of sea classification, when the model generates a false positive for a sea-related pixel, it implies that it mistakenly identifies certain pixels as valuable sea data despite they actually represent irrelevant data (clouds or land). However, this irrelevant pixel is not discarded nor degraded by lossy compression. Therefore, in the context of oceanic campaigns, the impact of the FPR is less severe than the FNR, as the FPR only results in a reduction in the efficiency of downlink usage, unlike the FNR which results in net data loss. This same analysis can be applied to land-focused campaigns. Namely, both the FNR and FPR continue to be the main metrics and also with a crucial relevance on the FNR due to the loss of relevant land data, similarly to what occurs in oceanic campaigns where the sea data is of main importance. 



% Based on the analysis above, we conclude that in the ranking system depicted in Figure \ref{Fig:flow_chart_ranking_system}, both for sea and land categories, the FNR takes precedence over the FPR. This is because higher FNR values result in a larger irreversible loss of important data, while higher FPR primarily impacts downlink efficiency but does not lead to the loss of valuable net data. Conversely, when dealing with cloud data, the critical metric is, however, the FPR. In this case, the FPR is associated with irreversible data loss, while the FNR is of less concern, affecting merely the downlink efficiency. In all cases, it is important to consider the FPR-FNR trade-off with their often inverse relationship \textcolor{blue}{as shown further in the subsequent results section}. 




% As depicted in the final part of the flow in Figure \ref{Fig:flow_chart_ranking_system}, we also establish a ranking system that prioritizes the HS images based on their significance, considering the sea, land, and cloud coverage levels. Consequently, beyond the false alarm ratios metrics presented above, we give special attention to evaluating the precision of the model's predicted rankings compared to the ground-truth rankings. For simplicity, we assess the model's ability to sort the images in queues based on three criteria: sea, land, or cloud coverage level. For each of these three cases, we evaluate how closely the model's predicted queue correlates with the true queue to determine the disparity in the image orders. Ideally, for each coverage level, the model should be capable of sorting the images in the same order as the ground-truth queue. To quantitatively assess the alignment between predicted and ground-truth ranks, we employ the Spearman's rank correlation coefficient. Instead of computing the correlation over the numerical image identifiers, which could yield misleading results, we calculate the coefficient based on the orders of the images in the predicted and ground-truth queues. The calculation of the Spearman's coefficient is as follows:


% \begin{equation}
%     \rho = 1 - \frac{6\sum d_i^2}{L(L^2 - 1)},
% \end{equation}


% \noindent where $\rho$ represents the Spearman's rank correlation coefficient, quantifying the degree of alignment between the predicted queue and the ground-truth queue. Here, $d_i^2$ consists of the squared distances between pairs of entries in the predicted and ground-truth queues, while $L$ denotes the equal length of both queues. The coefficient incorporates a scaling factor of 6, which is derived from the formula to normalize the rank differences, thereby constraining $\rho$ within the range of [-1, 1]. Specifically, $\rho$ serves as a quantitative measure of the monotonic relationship between the queues. Namely, a value of $|\rho|=0$ signifies no monotonic relationship, whereas $|\rho|=1$ denotes a perfect monotonic relationship, indicating a perfect match between the predicted and ground-truth ranking queues.


% While Spearman's coefficient provides insights into the performance of the queuing system when sorting images based on downlink priority, we recall that metrics like the presented FPR and FNR remain essential for assessing the ratio of data loss and downlink efficiency, as previously discussed. In addition to these key metrics, we also compute other additional metrics to gain further insights into the model's performance. Specifically, we approach the prediction of each individual coverage level, derived from the segmentation model, as if it were an individual regression problem. Namely, we calculate the Mean Absolute Error (MAE), a common metric in regression-based tasks, for each of the three coverage levels across the test subset. This involves comparing the predicted coverage level to the corresponding ground-truth level. Beyond the MAE, we make use of additional pixel-level metrics that are standard in the HSI segmentation field: overall accuracy, average accuracy, and the F-1 score, as detailed below:

% \begin{equation}
% \text{O.A.} = \frac{\text{NCP}}{\text{TNP}}
% \end{equation}

% \begin{equation}
% \text{A. A.} = \frac{1}{\text{NC}} \sum_{i=1}^{\text{NC}} \frac{\text{NCP}_{\text{class}} \times i}{\text{TNP}_{\text{class}} \times i}
% \end{equation}


% \begin{equation}
% F_{1} = \frac{2 \times \text{Precision} \times \text{Recall}}{\text{Precision} + \text{Recall}}
% \end{equation}

% \noindent where $\text{O.A.}$, $\text{A.A.}$, and $F_1$ denote respectively the Overall Accuracy, the Average Accuracy, and the F1-Score. Accuracy metrics offer a simple method for assessing the model's performance, but they can be misleading when dealing with imbalanced datasets, as it is the case. Consequently, other metrics like the F-1 score are frequently employed in such cases. The F-1 score calculates the harmonic mean between recall, which measures the proportion of true positives correctly identified, and precision, which assesses the correctness of predictions classified as positive. In the equations above, $\text{NCP}$ and $\text{NCP}_{\text{class}}$ denote the number of correct predictions across all classes and for an individual class, respectively. $\text{TNP}$ and $\text{TNP}_{\text{class}}$ denote the total number of predictions across all classes and for an individual class. 




% %%% From dataset paper:
% % Commented out for next paper (it seems more relation with Compressive Sensing): and each spectroscopic sample in the acquired cube is coded as a two-byte unsigned integer, resulting in an uncompressed image of size about 157 MB. 



% %%% From dataset paper:
% % \subsection{Dataset Calibration: From Digital Number (Raw) to Radiance}
% % Commented out perhaps for other paper where we do include the REFLECTANCE: After radiometric calibration, we conduct a radiance-to-reflectance conversion, yielding Top of Atmosphere (ToA) reflectance for each image in the dataset following the approach described in~\cite{Bakken2023}, using the mean solar exo-atmospheric irradiance and Solar zenith angle to account for the significant atmospheric effects. 








% %%% From dataset paper:
% % \subsection{Ground-Truth Labels: Semi-Automatic Pixel-Level Annotation for Sea-Land-Clouds Classification}
% % Commented out / Move it to GitHub (Radu): for each labeled image, we store multiple files that enable future adjustments to the labels if necessary. One of the most important exported files has the extension .dat, and contains the exported numerical labels. 
% %To ensure consistency with our desired class representation (starting by 0 for sea, 1 for land, and 2 for clouds), we use a custom script to adjust the output labels before saving and converting the ground-truth into a numpy .npy file, which can be easily loaded in Python.\\ 
% % Commented out / For next paper when we stop depending so much on labels: Despite the need for ground-truth labels in supervised learning and fine-tuning self-supervised pre-trained models, this labeling procedure has multiple downsides. One main disadvantage is its semi-automatic workflow, requiring human intervention to provide feature-extraction polygonal data for pixel-level classification. In contrast, DLNNs such as the one presented in Section~\ref{Section:METHODOLOGY_FCN} are fully-automated predictive models, automatically extracting data features through multiple neural layers before classification. Manual intervention in the semi-automatic labeling procedure leads to additional downsides: it becomes highly time-consuming, requires HSI expertise for feature extraction, the particular labeling tool has its own limitations.\textcolor{blue}{\textbf{Consider image where the polygons are shown, or figure to clarify the workflow as this text may be boring to read}}. 








% \subsection{Example of a Supervised Deep Learning Model: Pixel-Level Sea-Land-Clouds Classification by a 1D FCN}


% For the next paper: The initial feature-extractor block integrates four 1D convolutional layers with progressive kernel augmentation (size 3). The network's dense output layer computes class probabilities. 
% For the next paper paper - I'm not mentioning the other metrics nor the confusion matrix - but the confusion matrix should be given at least on GitHub or here if there's any space
% Commented out for perhaps next paper: from the trained model we can produce pseudo-labels that will be ground-truth












% \vspace{-5pt} % Jon from Dennis to reduce space
\section{NOT PART OF THIS PAPER . Extended State-of-the-art Review for the PhD thesis}

\jon{Commented out the extended state of the art to avoid that citations appear in the manuscript.}




% \subsection{Cloud Detection in Multispectral and Hyperspectral Satellite Imagery by AI: Advancements and Challenges}



% We conduct an extensive examination of the State of the Art (SoA) with emphasis on cloud detection from RGB to MSI and HSI satellite imagery aiming to identify unaddressed areas in the present literature, at the time of writing. We place significant emphasis on HSI due to the growing prevalence of satellite missions equipped with onboard HSI capabilities. In recent years, missions like ESA/Phi-Sat-1 \cite{esposito2019orbit} (European Space Agency), ASI/PRISMA (Italian Space Agency/PRecursore IperSpettrale della Missione Applicativa) \cite{cogliati2021prisma, cosmo2014future} and NTNU/HYPSO-1 (Norwegian University of Science and Technology/HYPerspectral small Satellite for Ocean observation) \cite{grotte2021ocean} have emphasized the importance of HSI for Earth observation. Furthermore, upcoming missions, such as ESA/CHIME (Copernicus Hyperspectral Imaging Mission for the Environment) \cite{nieke2018towards}, the forthcoming ASI/PRISMA Second Generation \cite{ansalone2023prisma}, scheduled for launch in 2025 by the Italian Space Agency according to \cite{spiller2022wildfire}, and the NTNU/HYPSO-2 mission planned for a potential launch in summer 2024 followed by the NTNU/HYPSO-3 mission \cite{langer2023robust}, all serve to highlight the relevance of HSI satellite technology for Earth observation, both in the present and in the future.


% We are in an era marked by significant hardware advancements that have revolutionized computational resources, facilitating the practical implementation of computationally-intensive AI techniques. This has resulted in a profound transformation of various industries, including the space sector with access to readily available and cost-effective Commercial off-the-shelf (COTS) hardware platforms \cite{giuffrida2021varphi, kothari2020final, furano2020towards, girshick2015region, spiller2022wildfire}, that are well-suited for deploying software for distributed edge computing AI algorithms directly at the data source. While traditional on-board processing hardware has historically depended on old components with limited computational capabilities \cite{furano2018roadmap, esposito2019orbit}, ongoing efforts are dedicated to incorporating satellite data processing platforms with significantly enhanced computational capacities. The current SoA extends from the cutting-edge Tensor Processing Units (TPUs) pioneered by Google and now being explored for space applications \cite{giuffrida2020cloudscout, jouppi2017datacenter, lotti2022deep} to the broader spectrum of Graphics Processing Units (GPUs) \cite{giuffrida2020cloudscout, nickolls2010gpu} tolerant to space radiation \cite{bruhn2020enabling}, Field-Programmable Gate Arrays (FPGAs) fabric logic integrated with System-on-Chips (SoCs) \cite{giuffrida2020cloudscout, dinelli2019fpga} \textcolor{blue}{resistant to the radiation?? [HYPSO-1 ref???]}, and Video Processing Units (VPUs) \cite{giuffrida2020cloudscout} tested not only in the Phi-Sat-1 mission \cite{esposito2019orbit, giuffrida2021varphi} but also in the International Space Station \cite{dunkel2022benchmarking}, as discussed in detail in \cite{antonini2019resource}. Additionally, the survey presented in \cite{li2020survey} provides an in-depth overview of various hardware accelerators, such as Intel's Neural Compute Engine, Qualcomm's Artificial Intelligence Engine (AIE), MediaTek's AI Processing Unit (APU), and HiSilicon's Neural-network Processing Unit (NPU), all meticulously optimized to enhance AI operations. 


% Initially proposed in \cite{esposito2019orbit, kothari2020final, furano2020towards}, the development of on-board Deep Learning Neural Networks (DLNNs) on COTS platforms is on the ascent, taking advantage of the repetitive operations such as multiply-accumulate (MAC) operations, and the structures inherent in DLNNs. At the same time, optimized reconfigurable COTS ensure minimal latency \cite{giuffrida2021varphi} and robustness against the lower total ionizing dose (TID) experienced by low-earth orbit (LEO) satellites compared to those in Geostationary Earth Orbit (GEO) \textcolor{blue}{[ref?]}. AI's capacity to derive highly valuable insights from data makes data a foundational and crucial resource nowadays \textcolor{orange}{PGK: This last sentence about AI deriving highly valuable insights sounds more like the motivation}. As a matter of fact, experts argue that data is potentially surpassing in value precious natural resources like oil. In contrast to oil, data possesses an inexhaustible production capacity. However, it parallels oil in that raw data, like crude oil, lacks value until it undergoes processing to unlock its potential worth. Just as oil's value escalates through refinement, data also gains value when processed, and unlike oil, it can be processed in multiple manners repeatedly accumulating additional intrinsic value. Therefore, the space sector also incorporates the mentioned AI techniques to process its data and extract this intrinsic informational value, concurrently diminishing the necessity for conventional on-board pre-processing and post-processing methods \cite{giuffrida2021varphi}.


% Following the satellite data revolution by the Copernicus Earth Observation Progamme, since around 2019 AI techniques have been experimentally deployed for the first time in space on the LEO Phi-Sat-1 mission for edge-based inference of in-orbit DLNNs, permitting for updates while the satellite is in orbit \cite{esposito2019orbit} for their on-board CloudScout DLNN model \cite{giuffrida2020cloudscout, pitonak2022cloudsatnet}. This in-flight reconfigurability allows approaches such as delta training, where only partial updates are made to some DLNN layers rather than to the entire model parameters \cite{giuffrida2021varphi}. The 6-U satellite, part of the ESA EOP initiative, is equipped with the HyperScout-2 push-broom imager which scans the Thermal Infrared (TIR) range from 8.0 to 14.0 $\mu m$ with 3 bands \cite{giuffrida2021varphi}. Additionally, the imager employs filtering via HS optical components across the Visible and Near-Infrared (VNIR) spectrum from 400 to 800 nm, featuring a spectral resolution of about 12 nm and 45 bands and acquiring the HS images using a Complementary metal–oxide–semiconductor (CMOS) sensor \cite{giuffrida2021varphi}. The collected experimental data, pre-processed from L0 to L2a calibration deviating from the the conventional approach of downlinking raw data, plays a pivotal role in AI-powered object detection by DLNN, which is essential for various change-detection applications such as recognizing plastics in oceanic environments, monitoring the health of vegetation, detecting wildfires, assessing fire risks, and issuing timely warnings \cite{esposito2019orbit}. For instance, this holds particular significance in safeguarding water systems vulnerable to Harmful Algae Blooms (HABs), which can have adverse effects on drinkable freshwater sources, as well as in protecting marine ecosystems that house sensitive fish farms prone to rapid marine fluctuations [HABs in fresh waters and also affecting fish farms]. However, the primary objective of the Phi-Sat-1 mission's initial phase is cloud detection in HSI \cite{giuffrida2021varphi}, a task that can be reliably and accurately accomplished using AI algorithms as highlighted in \cite{giuffrida2021varphi}, with a cloud coverage level surpassing 70\% at the image level serving as an indicator of a completely cloudy image. Cloud detection enables functions like cloud screening, a process specifically devised to eliminate and discard data obscured by clouds prior to its transmission to the ground, as explained in \cite{giuffrida2021varphi}. An alternative approach for handling cloudy-pixels data draws upon the concept of entropy from information theory. Entropy provides a lower limit for the efficiency of data stream compression by an encoder \cite{gray2011entropy, carter2007introduction}. In the case of encoding cloudy pixels, it is possible to use fewer bits than the intrinsic entropy of the data source, resulting in a deterioration of the quality of these superfluous cloudy pixels. Previous studies \cite{lebedeff2020board} have consequently introduced such selective HSI compression techniques in the spatial domain. These methods do not discard cloudy data but instead reduce the bit rate to degrade cloudy pixels while preserving the rest of the pixels. This can be achieved through the use of data compression methods such as CCSDS-123.0-B-2 \cite{hernandez2021ccsds}, which supports both lossless and near-lossless compression. In our prior publications \cite{justo2022comparative, justo2022study}, we have conducted assessments of alternative strategies to data compression techniques, including the utilization of Compressed Sensing (CS) in conventional HSI imagery. In this method, the need for an onboard compression algorithm is eliminated since compression is achieved through random sampling, thereby shifting the computational burden to the ground-based decompression and reconstruction phase, where we assumed the sparsity of the HS images after transforming them within the spectral domain.


% In addition to the Phi-Sat-1 mission focusing on cloud detection, other subsequent research \cite{salazar2022cloud} introduce a prioritization system ranking the images based on the detected clouds. This system determines downlink priority by evaluating the image cloud coverage level, calculated using cloud masks generated by CNN-based networks implemented on COTS Microcontrollers (MCUs). In the case of \cite{salazar2022cloud}, the authors employ an RGB true-color image composite from Sentinel-2B MSI data [reference to Sentinel 2B] to train their model making use of a dataset with labels of merely cloud masks as given in \cite{park2020rgb}. We note that the processing for this true-composite from the MSI data is comparable to performing RGB inference, as \cite{salazar2022cloud} selects three color bands out of the available 13 bands in Sentinel-2B. Indeed, in \cite{salazar2022cloud} the model undergoes further testing within an unexplored data domain, which comprises RGB imaging data sourced from the FACSAT-1 satellite.



% In short, the SoA \cite{esposito2019orbit} actively recognizes the numerous advantages of on-board cloud detection. These benefits involve e.g. conducting on-board post-processing solely on useful data and transmitting only meaningful imaging data, image thumbnails with reduced spacial dimensions as in the FACTSAT-1 mission \cite{salazar2022cloud} or metadata  to the ground \cite{zhou2019edge,mateo2021towards,jin2019channel,denby2020orbital}. This strategy optimizes the utilization of the Shannon data capacity which can be transmitted over a communication channel subject to stringent technological constraints and radio spectrum regulations governing downlink bandwidth as well as other signal-to-noise ratio (SNR) limitations. This optimization is especially critical when transmitting data with substantial bandwidth demands, as is the case with HSI data containing extensive spectral context. Additionally, on-board AI minimises the latency between the data acquisition and the decision-making process \cite{giuffrida2021varphi}. This latency includes the onboard inference time, the time required to establish line of sight (LOS) between the satellite and the ground station, and the subsequent downlink time once the radio link is established. Furthermore, this results in higher platform autonomy \cite{salazar2022cloud, spiller2022wildfire, furano2020towards, wang2019satellite, raoofy2022benchmarking, ghiglione2021machine}, thereby enhancing spacecraft payload independence from ground control. This elevated level of autonomy can also extend beyond the satellite itself, potentially serving as a catalyst for triggering various agents within an observational pyramid \cite{Bakken2023, grotte2021ocean, dallolio2021satellite}, including airborne systems such as drones, water vessels, and more. As a result, it leads to cost-efficiency gains by decreasing the necessity for ground personnel to analyze the data, especially important for latency-sensitive tasks such as issuing early warnings.


% The SoA in satellite technology acknowledges the significance of advanced onboard processing capabilities not only for cloud detection \cite{esposito2019orbit}, but also for applications such as wildfire detection \cite{spiller2021analysis, spiller2022wildfire}. In the recent work \cite{spiller2022wildfire}, the authors introduce a CNN-based network for wildfire detection, addressing a multi-class problem comprising five categories: fire, smoke, burned areas, vegetation, and bare soil. They accelerate their solution using COTS hardware, including the Intel Myriad 2 VPU, Nvidia Jetson TX2, and Nvidia Jetson Nano. The experiments conducted in \cite{spiller2022wildfire} are centered on HSI PRISMA data, with a specific focus on the Australian bushfires in December 2019. PRISMA data is characterized by a wavelength range of [0.4-2.5] $\mu m$, spectral resolution below 10 nm, and a ground sampling distance of 30 m \cite{spiller2022wildfire} \textcolor{blue}{[ref to PRISMA (crosscheck numbers? / this should be in the intro of the missions)]}. Nonetheless, these capabilities encounter a major constraint, represented by the primary bottleneck of a limited power budget, which imposes restrictions on the satellite's processing capacity and hence COTS play a crucial role in the optimization of the ratio between computation workload and power consumption. The limitation in power budget is exacerbated by limited memory resources \cite{giuffrida2021varphi}, which makes the implementation of DLNN and CNNs on board challenging \cite{giuffrida2021varphi, liu2020deep, dai2019semisupervised, zhang2019remote}. This is despite the impressive performance of DLNNs in space applications, such as for scene classification, object recognition, change detection, and other remote sensing applications \cite{yang2010bag, girshick2015region, asokan2019change, zhu2017deep}. To compensate for the restricted power limitations, modern satellite platforms incorporate AI acceleration technologies beyond the traditional Central Processing Units (CPUs) and Graphical Processing Units (GPUs). Namely, missions such as Phi-Sat-1, utilizing the ``Eyes of Things'' (EoT) board \cite{deniz2017eyes} employ e.g. Intel's VPU (Movidius Myriad 2 Video Processing Unit), a technology found in millions of devices, also for advanced Computer Vision (CV) processing, and with a primary emphasis on achieving minimal power consumption, often below 2 W \cite{leon2021improving}, all the while maintaining rapid inference. In the literature \cite{giuffrida2021varphi}, additional considerations for selecting the Myriad 2 VPU include ensuring compatibility with the payload's form factor for seamless integration with sensors, reconfigurability, minimal heat generation, and support for high-speed interfaces. 


% Other missions such as HYPSO-1 \cite{langer2023robust} includes an on-board FPGA \textcolor{blue}{AMD/Xilinx Zynq 7030} (...)


% However, the existing body of literature \cite{esposito2019orbit} for Phi-Sat-1 emphasizes another significant challenge alongside the constrained power budget bottleneck: the limited availability of data for the training of onboard DLNN segmentation models, attributed according to the literature \cite{giuffrida2021varphi} to the fact that space agencies such as ESA produce for their missions new sensor technology and hence this produces different data domains which results in a lack of labeled ground-truth data and hence having to rely in many cases in synthetic data. This is recognised by the literature \cite{giuffrida2021varphi} to be a source of inaccuracy in the on-board inference results. For the Phi-Sat-1 mission, this challenge arises already from the data collected during the HyperScout-1 IOD mission \textcolor{blue}{[ref]}, which proved insufficient for effective training. To address this data limitation and emphasize the critical reliability of ground-truth labels for proper meaningful model training in e.g. supervised learning, we released an open HSI dataset, incorporating sea-land-cloud ground-truth labels in our prior publication in \cite{justo2023open}. Ensuring accurate model training, evaluation and testing for reliable on-board AI, is essential to prevent trained models from making erroneous or biased inferences resulting in an irreversible loss of valuable net satellite data \cite{giuffrida2021varphi}.






% \subsection{} %%% ARCHITECTURES (STILL NOT TRAIINING, EVALUATION, AND TESTING) 
% Cloud detection can be accomplished using various methods, including Machine Learning (ML) and the specific subset of DLNNs. Currently, DLNN algorithms are gaining prominence due to their neural architectures inspired by the human brain, enabling them to capture numerous complex non-linear relationships within data features. However, they come with drawbacks, such as being highly-parametrized models that result in increased complexity during training and inference, as well as larger on-board memory requirements. Additionally, DLNN models pose challenges regarding interpretability, often functioning as black boxes that make it difficult to understand and comprehend their decision-making processes \textcolor{blue}{[refs XAI]}. Next, we examine how recent literature addresses the optimization and compression of DLNN models for cloud detection in RGB, MSI and HSI satellite imagery by employing two distinct techniques: pruning, which involves trimming network layers and eliminating redundant neural connections and neurons without drastically compromising segmentation performance, and quantization, which focuses on reducing the binary discretization and precision of the model parameters.


% According to the literature \cite{salazar2022cloud}, the problem of cloud detection in satellite imagery has been previously addressed in RGB imaging using e.g. lightweight versions of U-Nets, such as LU-Net \cite{zhang2019cloud}, which utilize the red, green, blue, and NIR bands. \cite{salazar2022cloud} primarily focuses on NU-Net, a modified version of RS-Net \cite{jeppesen2019cloud}, itself a variant of U-Net \cite{ronneberger2015u}. RS-Net's effectiveness is evaluated using different band combinations in Landsat 8 images \cite{jeppesen2019cloud}. Multi-stream NU-Net is proposed due to its superior cloud segmentation performance in RGB images, particularly for image prioritization purposes \cite{park2020rgb}. Indeed, \cite{park2020rgb} demonstrates that the performance of the NU-Net tends to surpass LU-Net \cite{zhang2019cloud}, RSN-net \cite{jeppesen2019cloud}, as well as conventional ML classifiers like Support Vector Machines (SVMs) \cite{boser1992training}, Random Forest Classifiers (RFCs) \cite{breiman2001random}, and Gradient-Boosting Classifiers (GBCs) \cite{friedman2001greedy}. Notably, SVM performs less effectively than NU-Net in RGB images according to \cite{salazar2022cloud}. \cite{salazar2022cloud} also introduces the NU-Net-mod, a further refinement of NU-Net aimed at reducing the model's weight count as part of their model pruning efforts \textcolor{blue}{and using only a single band in both network streams} (architecture in Fig. 1 in \cite{salazar2022cloud}).


% %%%%%



% The literature suggests that reducing model size through pruning can also be accomplished by compressing CNN-based segmentation models using 1D convolutions, as opposed to the use of 2D convolutions. While 2D convolutions are standard in CV for HSI, where image data is typically partitioned into patches (tiles), there is a growing interest in the application of 1D convolutions for HSI tasks. This interest is driven by the need to process spectroscopic information, collected continuously along the spectral dimension in HSI data, as sequential data, somewhat resembling time series or text sequential data. Hence, the examination of 1D convolutions for this sequential spectroscopic data has experienced a surge in interest as indicated in [refs]. Similarly to unsupervised Self-Organizing Maps (SOMs) applied to HSI data clustering \cite{danielsen2021self}, 1D CNN-based models are relatively simple as they capture only spectral context, but they lack the ability to consider spatial context as other ML models based on ML/GBM in Phi-Sat-1 such as \textit{s2cloudless} \cite{zupanc2017improving, giuffrida2021varphi}, which is often crucial for accurate spatially coherent segmentation predictions in CV. However, in scenarios with limited power and memory constraints like satellites, the adoption of 1D convolutions is advantageous as it significantly reduces parameter count, while still maintaining satisfactory model performance and greatly diminishing both training and inference complexity. 


% This is the motivation behind our previous work in \cite{justo2023open}, where we illustrate the segmentation evaluation performance of a 1D Fully Convolutional Neural Network (FCN) comprising a 1D CNN structure for feature extraction from HSI data. Specifically, we made several adjustments to the hyperparameters of the network originally designed for soil spectroscopy-based clay content regression, as described in \textit{Liuetal} \cite{liu2018transfer} and later adapted for soil texture classification in \cite{riese2019soil}. In the context of spectroscopic soil texture classification \cite{riese2019soil}, the authors also trained and evaluated alternative network architectures, such as the one introduced by \textit{Huetal} \cite{hu2015deep}, which we observe being applied for wildfire detection in different works \cite{spiller2021analysis, spiller2022wildfire}, where the authors provide insights into the computational performance of different hardware setups \cite{spiller2022wildfire}. They report approximate inference times of 5.8 ms, 3.0 ms, and 3.4 ms, along with average power consumption figures of 1.4 W, 2.1 W (GPU only), and 2.0 W (GPU only) for the Myriad 2 VPU, GPU Jetson TX2, and GPU Jetson Nano, respectively. 




% %%%%%

% \subsection{} %%% Training, evaluation, and testing results

% As previously discussed, data forms the foundational basis for ML and DLNN algorithms. In supervised learning, having a reliable dataset with accurate ground-truth is essential to ensure the correct functioning and generalization of on-board ML and DLNN models for unseen data. To achieve reliability in the the dataset presented in our previous publication \cite{justo2023open}, we simplified the labeled categories focusing on the clearly defined classes sea, land, and clouds to ensure their accuracy when labeling the high-dimensional HSI feature space. While we initially considered including various water colors in \cite{justo2023open}, colors like green or cyan lacked concrete and definitive meanings and were insufficient for a strong and scientifically supported preliminary consideration due to the multitude of uncertain factors affecting water colors in the complex waters of the ocean such as the seabed characteristics and possible phytoplankton presence \cite{justo2023open}. To ensure accurate on-board AI and mission's accountability, reliable ground-truth and a structured plan for training, evaluation, and testing with standard metrics are vital. On-board algorithms must undergo thorough processes according to the plan, including e.g. hyperparameter tuning optimization. We explore next how current literature applies these procedures to cloud detection in RGB, MSI, and HSI satellite imagery.




% Concerning preprocessing, there exists a consensus within the literature on HSI cloud detection that recommends using a limited number of spectral bands. This approach aims to reduce both the on-board computational memory footprint requirements and computational power usage while maintaining acceptable performance levels. As an illustration, in the case of the Phi-Sat-1 mission \cite{giuffrida2021varphi}, dimensionality reduction through Principal Component Analysis (PCA) is performed on the ground to select three bands. This practice helps avoid implementing PCA on the satellite's CPU, which would otherwise increase power consumption. Consequently, in Phi-Sat-1, only three pre-defined bands are extracted directly from the acquired data cube. 



% Furthermore, to create room for additional layers, one potential strategy is to segment the data into non-overlapping or overlapping 2D patches. This approach aims to minimize the inta-layer memory footprint by significantly reducing the spatial dimensions of the input batch tensors and enabling the incorporation of more layers. For instance, in the Phi-Sat-1 mission \cite{giuffrida2021varphi}, HS images exhibit a spatial resolution of 1152x1152, while the patch size is reduced to 192x192. This reduction results in a patch map consisting of 6x6 patches distributed across the image. Consequently, when comparing the patch size to the original spatial dimensions, we observe that patching reduces approximately 83.33\% of the total spatial dimension before patching.



% As it occurs in the Phi-Sat-1 mission \cite{giuffrida2021varphi}, another possible preprocessing step involves normalizing the acquired data samples to a range between 0 and 1, where the normalization is conducted on 16-bit floating-point representation for the data samples, which is the available arithmetic format compatible with the CPU on board the Phi-Sat-1 mission and hence that the model parameters are also quantized as 16-bit floating-point arithmetic. 





% Metrics such as accuracy \cite{salazar2022cloud}, precision \cite{salazar2022cloud, spiller2022wildfire}, recall \cite{salazar2022cloud, spiller2022wildfire}, and F-1 score \cite{salazar2022cloud, spiller2022wildfire} are frequently calculated at the pixel-level for semantic segmentation tasks. Additionally, other metrics, such as Spearman rank correlation coefficients, are employed for assessing the predicted priority ranking level against the true priority level \cite{salazar2022cloud}.


% In the context of a cloud detection ranking system, \cite{salazar2022cloud} reports accuracy and F-1 score values of 0.91 and 0.83, respectively, evaluated on a dataset of 100 images from Sentinel-2B.




% Given the frequent deployment of new sensor technology, \cite{salazar2022cloud} conducts tests on the NU-Net and NU-Net-mod models using RGB data from an unseen domain. This domain is considered unseen because it originates from a different sensor imager. Consequently, metrics relying on ground-truth categorical labels, such as accuracy and F-1 score, are unattainable for this new data domain. As a result, the evaluation relies on qualitative assessments based on the authors' expertise in \cite{salazar2022cloud}. In order to facilitate inference with FACSAT-1 RGB data, \cite{salazar2022cloud} modifies its dimensions to match those in the interface of the NU-Net and NU-Net-mod models specifically tailored for MSI in Sentinel-2B.



% Model quantization is performed in some works such as in \cite{salazar2022cloud} and in the Phi-Sat-1 mission \cite{giuffrida2021varphi} where model parameter quantization is performed to convert them into a 16-bit floating-point format, ensuring compatibility with the mission's on-board CPU. In contrast, other works such as for wildfire detection \cite{spiller2022wildfire} based on the simple and small \textit{Huetal} \cite{hu2015deep} employ the default Keras data type of \textit{float32} and hence they do not need to make any quantization \textcolor{orange}{PGK: PGK mentions that model quantization was commented some paragraphs before}. 



% This suggests that our modified 1D FCN model based on \textit{Liuetal} and utilizing the \textit{float32} data type in \cite{justo2023open}, could potentially be suitable for on-board implementation on HYPSO-1's ARM Cortex processor, which is compatible with this data format. This is contingent upon conducting a preliminary resource analysis and considering model pruning as a potential optimization strategy.




 


% Popular frameworks include TensorFlow \cite{salazar2022cloud} for model development and TensorFlow Lite \cite{salazar2022cloud} for deploying models on resource-constrained mobile and embedded platforms.




% \subsection{} %% Critical 
% % To the best of our knowledge, (...)
% % CRISP-DM methodology
% % That the labels that salazar2022cloud uses for the ranking system are only for cloud detection and not for sea and land additionally. We can mention that we do notice that according to the spearman correlation coefficient in salazar2022cloud, the NU-Net-mod performs worse when it comes to the ranking according to cloud detction but however there are othber metrics such as accuracy and F-1 socre that perform slightly better --> there should be a mention to Dilip here regarding power consumption (C02 footprint) to just get a bit more decimals of model accuracy. 
% % We should really say that in salazar2022cloud, they do some quantization but that they do not conclude (we do it) with the conclusion that when comparing Table 4 and 5 in salazar2022cloud, we can see that althoguh quantization has played sopme effect, it's not fully critical at all and the change inhe metrics is mininal and absolutely acceptabøe. 
% % The fact that spiller2022wildfire does not make any quantization and they use the default dtype in Keras of float32, suggests the following: that our modified version of the \textit{Liuetal} trained model openly avaialble in \cite{justo2023open} (also in float32) may be preliminary and with caution considered as feasible for on-board of the HYPSO-1 mission (I say preliminary and with cuation since the number of parameters is over 100 000 - I think probably still feasible since it would be 400 kB - we could compute how many kB)  

% %% IMPORTANT: It should be clear that we present a system in general for HSI imagery and that HYPSO-1 is the use case of example to demonstrate how such system would work. 






% Commented out the next as it is too detailed. 
% Parameters for architecture and training the model <-- Commented out as it has many more details that might not be needed for this paper about the dataset
% \begin{table}[htbp] 
%     \centering 
%     \small
%     \caption{Details for Model Architecture and Training}
%     \label{Table:Hyper_parameters}
%     \begin{tabular}{cc} 
%         \toprule % Top horizontal line
%         \textbf{Parameters} & \textbf{Value}  \\
%         \midrule % Middle horizontal line
%         Input Dimension & $batch\_sizex114$ \\
%         Processing Type & Pixel Level \\
%         Conv. Kernel Size & 3 \\
%         Nr. of Kernels per Convolution & 32, 64, 96, 128\\
%         Dropout Layers & Disabled \\
%         Nr. of Trainable Parameters & 63.779 \\
%         Output Dimension & $batch\_sizex3$ \\
%         Output Type & Probabilities \\
%         Type of Learning & Supervised (one-hot enc. labels)\\
%         Optimizer & Adam \\
%         Loss Function & Categorical Crossentropy \\
%         Training Metric & Accuracy \\
%         Epochs & 1 \\
%         Batch Size & 300 \\
%         Validation set passed to .fit() & Yes\\
%         Framework & Keras \\
%         \bottomrule % Bottom horizontal line
%     \end{tabular}
% \end{table}


==> X-SOA_DRAFT_NOTES.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% IMPORTANT: DO NOT EDIT THIS .tex FILE
%%%            THIS .tex HAS DRAFT NOTES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% DISCUSSION BASED ON HIGHLIGHTED READING

% SMALLSATS APPS.:
%   Main application: Earth observation, first demonstration of smallsats for EO was around 2000. \cite{salazar2022cloud}
%   Concrete lower-granularity applications from \cite{salazar2022cloud}: wildfire detection \cite{spiller2022wildfire}, [[19] in ref \cite{salazar2022cloud}-CNN wildfire detection in cubesat], deforestation monitoring [ref?], ship detection [ref?], land use[ref?], surface water mapping. 
%   


% CHALLENGES IN SMALLSATS - AGREEMENTS WITH SOA: 
%   MASSIVE AMOUNT OF DATA (INCREASING - ANY REF ON HOW IT WILL INCREASE?)
%   DOWNLINK: SHANNON CAPACITY - LIMITED DATA RATE AND SPECTRAL LIMITATIONS BY REGULATIONS. RADIO RESOURCES USED INEFFICIENTLY DOWNLOADING IRRELAVENT IMAGES. 
%   STORAGE, TX, AND PROCESSING OF THE MASSIVE DATA
%    POWER CONSTRAINTS (ANY REF TO HYPSO-1 POWER?)
%    MEMORY FOOTPRINT FOR INFERENCE ONBOARD 

% AGREEMENTS ABOUT ISSUES FOR AI ONBOARD - WITH SOA: 
%  AI demands for power consumption, and processing speed ref \cite{salazar2022cloud}
%  Most works agree on the importance of proper HW platforms, and still it's resource-constrained and works such as ref \cite{salazar2022cloud} mention CNNs on GPUs for cloud segmentation in MSI (X: With HSI it would be even worse) [15 ref \cite{salazar2022cloud}]. Mention HW platforms ASIC, GPU, FPGA ref \cite{salazar2022cloud}. 
% ref \cite{salazar2022cloud} states that [18 ref \cite{salazar2022cloud}] proposes CNNs to select an image to downlink. 


% DISAGREEMENTS RELATED TOP AI ONBOARD - WITH SOA: 
%   RELATIVE RESULTS: Work ref \cite{salazar2022cloud} mentions that the accuracy of CNNs is lower due to quantization and pruning (define both terms). However, in works such as ZZ it is mentioned that the quantization didn't affect the accuracy, so this is very relative. Agreement: quantization and pruning are the techniques often used. 


% AGREEMENTS ABOUT CLOUD DETECTION WITH SOA:
%   Visible wavelengths are blocked due to clouds - in the NIR there can be also scattering and absorption but there's a stronger penetration compared tko the visible. However, for the visible wavelenghts there's some dominating scattering (and a bit of absorption). This limits many applications but there are still many small satellites focusing on the visible spectra, e.g.: HYPSO-1 (give range and I think it's [bakken2023firstimages], HyperScout-2 [\cite{esposito2019orbit}]), then PRISMA range is wider but with wither hiperspecrtal channel ("worse" spectral resolution) ref \cite{spiller2022wildfire} and ref [PRISMA original paper?]. 

% REGARDING CALIBRATION LEVELS: 
%   Refer to slack message from Marie from 07.09.2023 (Thursday) 12:45 PM from Level 0 until Level 2 (justo2023open is L1b). 


%% REGARDING SOFTENING EFFECT: 
% It can happen that there are sporadic misclassifications in the prediction, then we can use pixel similarity / spatial proximity techniques such as CRF (there's even a library for it in Python) - my guess is that this CRF could be on ground?

%% REGARDING THE FEATURE SPACE: 
% Remember the N-dimensional feature space. 

 
% REFERENCES FOR CLOUD DETECTION IN THE STATE OF THE ART - CRITICAL: 
%   \cite{salazar2022cloud}: Cloud detection, but in RGB images for priorization based on the cloud coverage level in percentage from a cloud mask produced by a CNN-based network, defining the downlink priority, CNN in COTS MCU (COTS is common), 100 testing images and with accuracy of 0.91 and F1 0.83. IMPORTANT: It's confusing that although they insist on RGB, it is indeed mentioned that Multispectral Images Table 3 are used, in particular, Sentinel-2B images with 13 bands but they mention that the "product used" from sentinel-2b is the "true color image" (so a composite) - check in 24 in ref \cite{salazar2022cloud} if it is mentioned what the dataset contains exactly since ref  \cite{salazar2022cloud} uses the dataset from the referred 24. Points to previous SOA solutions such as downloading thumbnails image (reduction of the spatial dimensions) and this is carried out by the FACSAT-1 mission [12 ref in \cite{salazar2022cloud}]. Agrees on automation onboard for cloud coverage by AI. Points to previous SOA and states that a lightweight version of U-Net proposed in [22 in ref \cite{salazar2022cloud}] with the name LU-net to detect clouds using 4 bands (R, G, B, and nearNIR). The variant of U-Net they actually focus on is RS-Net tested for different combination on bands in Landsat 8 images [23 ref \cite{salazar2022cloud}]. The reduceed version of this RS-Net is called NU-Net proposed for its good cloud segmentation performance but using RGB images for image prioritization [24 in ref \cite{salazar2022cloud}]; the peformance of the NU-Net is demonstrated in [24 in ref \cite{salazar2022cloud}] to be above the mentioned LU-net in [22 in ref \cite{salazar2022cloud} - check if indeed the ref is for the LU-net, it should be], and also above the RSN-net [23 in ref \cite{salazar2022cloud}], and over classifical RFC (forest), GBC (Gradient), SVM. IMPORTANT: They point SVM as demonstrated in RGB images to have lower performance compared to NU-net. Sequence: U-Net, simplified version is RS-Net and the NU-Net is based on the RSN-Net - NU-Net has a reduced number of kernels (remember pruning). They propose NU-Net-mod to decrease number of weights (pruning effort).  Points to issues in CNNs (Jon: probably not only CNNs) with unseen domains by the model, so they test the model also with a different data source too (the images changes the domain) - refer also to ESA's paper pointing to new sensors for each mission. (X: NO HSI BUT RGB, extensive testing subset but ofc it's RGB not HSI, V: STILL MANY APPROACHES USE ONLY 3 BANDS AFTER DIM.REDUCTION). NU-Net and NU-Net-mod follow a multistream approach but the -mod uses a single band in both stream (not sure what this means). Ref to Fig. 1 in ref \cite{salazar2022cloud} for details on architecture. They use labels for cloud masking (RGB) to train the CNN from [24 in ref \cite{salazar2022cloud}]. Generalization: they use a different dataset from another differnt imager to see how well the model generalises for another unseen domain - there they don't have labels and the analysis has to be qualitative. The evaluation is applied to the RGB imaging from the FACSAT-1 mission with spectral response RGB (they actually adapt the spatial resolution of the RGB data from FACSAT-1) - NB: remember the training also includes multispectral but they a composite. Data augmentation is used (e.g.: rotation). LOSS: BINARY CROSS ENTROPY (Binary classification problem), optimizer: ADAM, learning rate: 1x10^-4, number of batches 10, steps per epoch 200, epochs 100. Metrics: accuracy, precision, recall, F1 score (relate to the evaluation of the predicted classes at pixel-level), and they use also the "spearman rank correlation coefficient" (related to the evaluation of the predicted priority level) (statistics) in page 5/19 in ref \cite{salazar2022cloud} to evaluate the "predicted priority ranking against the true priority rank" - check what this means but I think it means they take the % level of clouds (just the ratio in the image - 100 % fully cloudy) in the ground truth and then they have the ground-truth priority ranking, then they calculate the same but for the predicted labels and then they obtain the predicted priority ranking, and then the 2 rankings are compared using the spearman rank correlation coefficient (NB: Correlation). NB FOR HYPSO: The same could be done not just for clouds but also for priority ranking of sea (water bodies). Mention to Tensorlow to develop and TensorflowLite (I think often used to deploy on mobile platforms). IMPORTANT: Give same plot as in Fig.3 ref  \cite{salazar2022cloud}, a) level percentage of a class (ground-truth) in X, and then in Y we have the predicted level percentage and we can see the alignment with ideal case which is y=x (we can plot multiple classes, or multiple ML/DL architecutres), b) same idea but there we have the ranking of the images (it does give the impression that the NU-Net-mod performs worse which is later confirmed by the Spearman coefficient) - comment also on the outliers (any metric COMMONLY used to measure the outliers with respect to y=x). It's also possible to give the thumnails of the ranking in ground-truth and also in prediction so compare the sorting. Also, they do the same for unseen domain (and data) regarding the sorting (priority ranking) according to the cliud coverage level. X: In Table 4 it can be seen that the spearman correlation isn't better for the NU-Net-mod, also the pixel-level results are not improved - mention to the power consumption in AI and carboon footprint [Dilip]. In the paper, they mention that they implementy in an embedded device where they perform quantization, but they don't say clearly how the quantization is affecting (no need to mention this in our paper), we can then conclude that comparing Table 5 against 4 ref \cite{salazar2022cloud}, we can see that although quantization has played some effect it's not fully critical and the change in the metrics is minimal and I think absolutely acceptable. IDEA (ONLY POSSIBLE IF WE HAD THEIR TRAINED MODEL): Would it be possible to check if their model certainly generalizes well on HYPSO-1 for cloud detection? X: Where's the model? (lack of availability; dissemination problem addressed in ref \cite{justo2023open}. NOTE: They give the data availability at the end. 


%% \cite{spiller2022wildfire}: this one is for HSI data (PRISMA) and for wildfire detection. They insist on "edge computing" (this is the term they use) (inference at the edge) for the CNN to stengthen the "COMPUTING CAPABILITIES" AND HENCE THE "PLATFORM AUTONOMY. They point that there's an increasing interest in edge computing based on AI methods [4-7 in ref \cite{spiller2022wildfire}]. In the case of PRISMA the range is [0.4, 2.5] microm and spectral resolution less than 10 nm (JON: figure out how much exactly), ground sampling distance is 30 m for PRISMA. X/V?: we should highlight any benefit of HYPSO-1 over PRISMA data as it could be claimed that PRISMA is providing a larger spectral range and especially larger in the NIR which is important when having clouds since NIR tends to penetrate more (JON: again these depends on the wavelengths in the NIR, and also the compsition and thichness of the clouds). The paper is for a particular event: Australian bushfires in December 2019. The platforms used as HW acceleration are: Inel Movidius Myriad 2 (IMPORTANT), Nvidia Jetson TX2, Nvidia Jetson Nano. Insists on the common approach to have COTS such as in Phisat-1 for on-board cloud detection [refer here to \cite{esposito2019orbit} and \cite{giuffrida2021varphi}], and also in other missions such as HYPSO-1 using low-cost COTs components as stated in ref [D. Langer].They mention as future missions CHIME and they give for it the reference [23 in ref \cite{spiller2022wildfire}] and even a PRISMA Second Generation declared to be launched in 2025 by the Italian Space Agency ref \cite{spiller2022wildfire}. X: They only use one image from PRISMA and that image is used for training and testing - refer here about this issue addressed ref [justo2023open]. The CNN they use is 1D FCN and is the based on the Huetal  in the list from Felix about soil texture [find ref], the Huetal [ref here to Hutetal which is 25 in ref \cite{spiller2022wildfire}]. That network based on the Huetal was used by the same main author previosly used in [14 in ref \cite{spiller2022wildfire}]. X· Issue not spatial context and possible misalignment and not given a metric to justify such decision. NOTE: You can use a framework for development and usually there are other steps involved for the deployment phase of the mode. NOTE: For the training they used Nvidia RTX2060 (just curious to check if our GPU is more powerful-I think so). The metrics reported in Table II ref \cite{spiller2022wildfire} are precision, recall and F1 - X they miss the accuracy but ok, we don't have to say that I guess; X: although they do report on the test set, the problem is that this is for the same scene which is not realisitic (what I would argue is that the data used for testing and for measuring for metrics are based on a "non-varied" data), e.g.: what if a fire in a different scene with a different exposure setting?. IMPORTANT RESULTS ABOUT THE SPEED OF INFERENCE ON THE MENTIONED PLATFORMS and gives as ref Table III in ref \cite{spiller2022wildfire} - THESE ARE THE 2 MAIN PARAMETERS THEY ANALYSE: INFERENCE TIME + POWER CONSUMPTION.  a) MOVIDIUS: approx. 5.8 ms and computational average power of 1.4 W, b) Jetson TX2: approx. 3.0 ms and the average computational power is 4.8 W (2.1 W if considereing the power consumed by the GPU only), c) Jetson Nano: approx. 3.4 ms and the average computatonbal power is 2.6 W (2.0 W if considered the popwer consumed by the GPu only). JON/CONCLUSION: I think it would be worth to prioritize the Movidius as they indeed offer a smaller consumption and saving as much as power as possible it's important and the increase in ms is absolutely acceptable. NOTE: Weights are in float 32 (this is indeed the default type in Keras and used by other works) [justo2023open] - these power consumptions is in line with space mission according to ref \cite{spiller2022wildfire}. As mentioned later on, they will not make any quantization due to the simplicity of the model - they have not reported which evaluation metrics they get in the devices, but I would assume that since the model parameters have not been changed at all, then this is why they don't mention these metrics on the devices (although they should have) - I think it's a correct assumption to say that for Movidius then the evaluation performance compared to the other 2 GPUs is the same stengthing the conclusion that Movidius would be better. ALSO, IMPORTANT TO HIGHLIGHT THE SHORT TIME USING MOVIDIUS.   IMPORTANT: In this case they use the adam, and also they use CATEGORICAL CROSS-ENTROPY so we are in front of a multi-class classification problem with 5 classes: 0-fire, 1-smoke, 2-burned, 3-vegetation, 4-bare soil. V: Great, training for more classes, X: only for 1 image and this is very limited; if they tried to expand that to more images they would need plenty of efforts and challenges to build the labeled dataset as in ref [justo2023open], and also they would face questions about the reliability of the labels (the more categories, the more challenges can show up on the way) - for one image is ok, another story is for 38 images as in ref [justo2023open]. Mention to GPUs being radiation tolerant in space [26 in ref \cite{spiller2022wildfire}] and the Movidus (VPU) has been tested not only for the Phisat-1 mission [give 2 citations to Phisat-1 here] but also in the International Space Station [27 in ref \cite{spiller2022wildfire}]. For Movidus, they mention that the Keras model can be transforrmed to an OpenVino format accpmplshed through the use of the OpenVino Intel library for HW optimised comutere vision typical in Intel processors and known for being "extremely easy to use" according to ref \cite{spiller2022wildfire}. IMPORTANT: Since the CNN model was small, they didn't have to do any quantization of model parameters- remember: quantization and pruning efforts. OTHER PLATFORMS MENTIONED: Google Coral TPU or FPGA SoCs. 



%% \cite{esposito2019orbit}: no results in this paper, it is just a GENERAL DESCRIPTION on the Phi-Sat-1 mission - details: part of the ESA EOP initiative - and this sat is also a 6U as HYPSO-1 [ref HYPSO-1]. NAME OF THE IMAGER: HyperScout-2 scans the TIR (thermal IR) and the VNIR 400-1000 nm and with a spectral resolution of 12 nm - I cannot see how many bands in the VNIR but in ref \cite{giuffrida2021varphi} it is mentioned that it's 45 bands from 400 to 1000 nm (this is the most updated version; however taking into account the article esposito2019orbit my calculation would be that 50 bands are used instead)(V: HYPSO-1 smaller spectral range but finer spectral resolution); in  the case of the TIR the spectral range is 8.0-14.0 \microm in 4 bands (it is mentioned 3 bands in ref \cite{giuffrida2021varphi} which is more updated). Processing platform has: CPU, GPU, and VPU (from Intel) (Movidius Myriad Video Processing Unit VPU - Movidius is actually an Intel's company) and typical for vision processing. HyperScout-2 will capture experimental data for use in AI for multiple applications that can benefit from object detection and data inference, and this first application will be cloud detection - they mention that they have selected this application since the clouds is one of the fundamental problems in optical remote sensing. JON: they use the term "cloud screening" as way to refer not only to the cloud segmentation, but also to their exclusion (remember that another approach would be to change the data rate for the cloudy pixels as done in ref \cite{lebedeff2020board}). Goal: high processing capability in orbit. Challenge: limited power and challenge to download the large amount of data acquired omnboard and its processing. They mention that they ACQUIRE THE DATA + L0-L2a + NN INFERENCE FOR CLOUD DETECTION. BENEFITS OF CLOUD DETECTION: Content of the downloaded data and latency, downlink, power, and operational costs (JON: automation/platform autonomy - independence of the of the spacecrafts and payloads). APPLICATIONS OF AI ONBOARD: Plastic detection on the sea surface, vegetation conditions, fires, ajd early warnings (remember HABs). They mention that there are application that can benefit especally from having AI omboard: related to change detection for instance (AQUACUTLURE - CHANGES IN THE MARINE ENVIRONMENT AND HOW THE FARMED FISH RESPONDS TO THE CHANGES). It also allows to apply data post-processing onboard only to the useful data; they mention again the application about the risk assessment for fires (remember the wildfire paper). LATENCY: INFERENCE TIME + DOWNLINK TIME. I will copy-paste what they write about algae blooms: "Another interesting application is the detection of Algae blooms in in-land water bodies used for the production of drinking water, for which the detection of such a phenomena early in the process can lead to have a large financial saving.". The following is A SUPER IMPORTANT PARAGRAPH THAT SUMMARISES WHY AI ONBOARD: "PhiSat-1 will be the first demonstration of in-orbit neural network inferencing performed on newly acquired data. The combination of on-board processing and inferencing for object detection and/or near real time information extraction is a turning key for small satellites constellations, which would depend less and less from the ground crew to analyse the data for early warning and operational activities which require low latency between the acquisition and the information usage. All this also relaxes the downlink necessities, which for small satellites is often the bottleneck." Regarding the low latency is the time between the observatio and the decision making process/information usage (JON: this can trigger further devices in the pyramid). They insist on the low-power consumption of the Movidius and still high performance. They mention that m illions of devices with Myriad 2 on the market today are found and also very much for AI (imaging processing and CV tasks). They highlight the fact that they the platform can be updated during flight [ref also to HYPSO-1]. Advantages of SmallSats: lower costs for development and launch. They mention that the revolution in satellite data usage was brought by the Copernicus Earth Observation Programme. They mention that one of their problems to implement the CloudScout (this is the model) is the lack of sufficient data for training since the data downloaded during the HyperScout-1 IOD mission was not sufficient to be used for training (refer to [justo2023open]). 




%% \cite{giuffrida2021varphi}: insists Phi-Sat-1 is the 1st NN onboard (exeperimental) to demonstrate DNN inference on COTS to reliably detect clouds on acquired HS images. Insists on the extraction of the relevant features from the data. They use the term ratio between computation and energy consumption, and AI algorithms at the edge. Mentions the meaningful and useful data and hence minimizing the required data bandwidth and reducing the latency. They mention AI is reliable and accurate for cloud-detection in an HSI mission. They mention the CloudScout segmentation NN running on Myriad 2: identify + classify + discard on-board the cloudy images (cloud screening as mentioned in ref \cite{esposito2019orbit}). Increase of more "private ventures" in addition to public sector agencies (so more data produced). Mentions that on-board processijng still relies on old components and hence not providing enough computational power to run innovatie algorithms as in [4, and 5 in ref \cite{giuffrida2021varphi}]. They mention that AI reduces the standard on-board preprocessing and post-processing techniques. It insists on the limited computatonal power and memory resources constraints and that CNNs and DNNs suffer from a challenge to be implemented there according to [7-9 in ref \cite{giuffrida2021varphi}]. They mention the COTS and that the total ionizing dose (TID) for low earth orbit (LEO) misssions is much less than for Geostationary Earth Orbit (GEO); JON: HYPSO-1 is LEO. NB: Phi-Sat-1 is also LEO, and NB that is for EO. They board including the Myriad 2 version is called "eyes of things (EoT) [15 in ref \cite{giuffrida2021varphi}] [I have also seen that EoT by Castilla la Mancha is in [9] in ref \cite{giuffrida2020cloudscout} but I haven't checked if it's the same reference as [15] in the refered work, I would guess so?] while pointing to the fast inference and a power consumptio well below 2 W [16 in ref \cite{giuffrida2021varphi}]. It is also mentioned the parameters they consider for choosing the Myriad, which are: payload-compatible, host-controlled, reconfigurable,. low power, low heat generatiuon, high-speed inerfaced device, in a form-factor to integrate well in the sensor payload. X: Although thyey mention about AI handling raw L0 data or L0 to L1 data on-board, they don't make a comparison on such stage would affect the cloud detection. X: they insist on the lack of training data and hence they dad to synthesize images starting from the Sentinel-2 dataset [19 in ref \cite{giuffrida2021varphi}] to emulerate the new camaera sensor characteristics and then using the result for training and testing. Percentage of cloudy images less than a given threshold. COTS advantages: distributed edge compoute at source (so, several units working in parallel subtasks) and they deliver low latency, the reconfigurability of the NNs for instance for delta training (the NN isn't trained from scratch), COTS enable also more processing capabilities since the traditional approach was to downlink raw data but now we can preprocess it and even calibrate it on-board. DNNs have shown in space applications remarkable results such as scene classification [22 in ref \cite{giuffrida2021varphi}], object recognition [23 in ref \cite{giuffrida2021varphi}], change-detection [25 in ref \cite{giuffrida2021varphi}], and others [26 in ref \cite{giuffrida2021varphi}]. Benefit of AI onboard: transmit to ground only useful data or meta-information [27, 28 in ref \cite{giuffrida2021varphi}] and this can relax bandwdth reqirements by filtering out nonuseful data [2, 29 in ref \cite{giuffrida2021varphi}]. See what they literally say about ensuring the reliability of AI onboard: "reliability of the processing is of importance since a false detection can lead to an ULTIMATE AND DEFINITIVE LOSS OF DATA". They mention that porting DNNs on board spacecrafts using particularly COTS HW accelerators for inference was proposed by [17, and 1 in ref \cite{giuffrida2021varphi}], and also that COTS can exploit the repeated execution of the same type of building block operaitons such as MAC operations, and that these COTs have a great market access and reduced costs with reference again to [1, 17, and adding 23 in ref \cite{giuffrida2021varphi}]. It mentions that the sensor is used in push-broom mode "exploiting the orbital motiuon of the satellite for the acquisiiton" of the data. Easy how the camera is described: CMOS sensor + hyperspectral FILTERING element to separe the wavelengths. It's interesting to see that they give a flat map for the world and then mark with points the geographical regions of the captures - I think this is certainly a way to compress the information about continents I initially tried to give in justo2023open. It's important to mention that they acknowledge that it's very common for instance in ESA mission to have new sensor technology producing new data domains and hence that there's a lack of data for the construction of dataset and ground-truth and hence having to rely on synthetic data anbd consequently they indeed mention that "the author appreciate that this is a potential source of inaccuracy in the in-flight inference rsults". They mention to SOA about "s2cloudless" [32 in ref \cite{giuffrida2021varphi}] as an ML cloud-detectuion algorithm, which doesn't take into account the spatial context, based on gradient boosting machine in Sentinel-2 imagery (X: Sentinel 2 is all MSI right? Not HSI). For the probablistic confidence map you can take the pixels that are decided to be clouds, and if the maximum probabily is of above a certain probability threshold then you assume it's certainly a cloud - another alternative is that instead of taking the max probability and infering the categorical class, you can just sert thresholds depending on the sensitivity of the model <-- IMPORTANT SINCE THIS MIGHT CHANGE THE RESULTS MUCH I THINK. I think they use a threshold of 40% and then if it's considered a "fully cloudy image" when the threshold is above 70% (regarding the 70% I'm very sure, but regardin g the 40% if not fully sure if it refers to the probabiliyt, although I think so - just take the 70% as reference to declare an image as fuly cloudy). THEY DO NOT PROCESS ALL BANDS -> IT WOULD TAKE MANY RESOURCES: MEMORY AND ENERGY --> THEY USE PCA TO PICK 3 BANDS (IT MIGHT BE USEFUL SO THAT WE CAN THEN USE REGULAR PRE-TRAINED RGB MODELS) --> POSSIBLE TO IMPLEMENT THE MODEL IN THE CPU BUT TOO DEMANDING IN TERMS OF POWER CONSUMPTION SO THE BEST IS JUST TO TAKE THE 3 BANDS FROM THE ACQUIRED CUBE AND DON'T RUN PCA ON-BOARD. IMPORTANT TOO: THEY NORMALIZE [0,1] AND 16-BIT FLOATING POINT FOR THE IMAGES (NB: NOT FOR THE PARAMETERS). In the case of Fig.6 in ref \cite{giuffrida2021varphi}, it's seen that most of the images either are cloud-free or fully cloudy and that might help define the threshold, in the case of HYPSO, I'm unsure if this categorical statement could be a valid approximation too. Each mission has their own band codes, and this is why the authors use the one for Sentinel-2 where the most sensitive bands for the cloud ndetection in the HyperScout2 are B01, B02, and B8A (450, 494, 862 nm, respectively) from the Sentinel-2, more info on bands (super importat as it tells you also for what each band can be used): https://custom-scripts.sentinel-hub.com/sentinel-2/bands/. It's very valuable how they explain the encoder-decoder architecture (the present a custum CNN-based NN for Phi-Sat-1 known as CloudScout and isnpired by U-Net [25 in ref \cite{giuffrida2021varphi}]): "A semantic segmentation network (see Fig. 9) is generally composed of two parts: encoder and decoder [33 in ref \cite{giuffrida2021varphi}]. The encoder extracts only the most relevant features from the input image and propagates them through the entire network, increasing the level of details within each feature. At the end of the encoding phase, a nonhuman-readable vector is extracted that captures a compressed version of the input image. This vector is input to the decoder, and, helped by the concatenation with the same dimension encoder layers, reconstructs only the most valuable information, creating the segmented images." - JON: the what and the where in encoder / decoder architecturs. Referto Fig.10 for the architecture - deconv layers used for upsampling. It is possible to halv the spatial dimensions using a stride (2,2) at the end (I wouldn't do so) to get a thumbnail - V: processing, tx, storage, but X: loss of detail. Mentioned to particular attention to convolution/deconvolution layers as well as intra-layer memory. NB: The memory during inference execution is the MEMORY FOOTPRINT. 16-bit floating point is the arithmetic available in CPU - they mention that they do quantization of the weights to 16-bit floating point. NB: 3 bands used as input - the spatial dimensions of the input tensor can also be reduced with the goal of having more space for layers; NB that the spatial resoluton they use is quite small 192x192 - they work at patches level (also referred as tiles level). IMPORTANT / PATCHING: Although they don't say it directly since they point that the 17 images in their data have a spatial resolution of 1152 x 1152 and the input to the network is 192x192x3, then it means that the patch map is 6x6 with each patch being 192x192 (then we can calculate ourselves that the patch size is approx. 16.67% of the spatial resolution so this means that the remaining pixels which are the difference that are not used is 83.33% - crosscheck reasoning). Training: BINARY CROSS ENTROPY, LEARNING RATE STARTS FROM 0.01, AND THEY USE THE ADADELTA OPTIMIZER INSTEAD OF ADAM (I guess these optimziers are different?). Epochs: 78 but they mention a patience of 4. They mention about the patch level (I guess they use then patching). The use also the ROC with TPR and FPR where the FPR has much importance. Regarding the reliability of detecting as cloudy things that are not cloudy means a "net loss of good data". The ROC is often for binary classification but we can one ROC curve per class and the curve is for different thresholds (each gives 1 TPR and 1 FPR). NOTE: The analysis authors make after TABLE II and TABLE III are important since the analyze the false positive rate and we should have a similar analysis. NOTE: They list in a table the metadata of their 17 images n addition to a figure with bars where they show the percentage of saturated pixels - they point saturation due to "bright clouds", and shwow in a figure the RGB composite for some of them. IMPORTANT: The inference time of the DNN (remember that DNNs are many times more complex than ML) is approx. 102 ms in the Myriad 2 and with a 62.9 KB of memory footprint. ALIGNMENT CHECK / IMPORTANT: after Fig.15 they give the analysis for the misaligment, this is important to address and measure since 1D approaches will suffer especially from this and also 2D approaches - [refer to Jonathan's thesis mentioning misalignment in HYPSO-1]. 2D approaches, as they take into account the spatial context, they can compensate a bit, however 2D approaches imply more comp. complexity and parameters. The misalignment can be measured, are there are indeed algorithms to do so. AWGN noise is mentioned, and this can indeed serve as a data augmentation technique, however the additive noise should be realistic (I wouldn't go for this in HYPSO-1 since the noise should be properly categorized - out of the scope), but the fact that even the authors are adding these noise is due to the efforts to produce more data to train the algorithms [justo2023open]. Although it's out the scope, they mention that the run also tests on the network inyYOLO [36 in ref \cite{giuffrida2021varphi}] for object detection. 

%% \cite{lebedeff2020board} - NB: I don't like at all that they are using an excessive amounts of URL/I'd rather replace the citations by articles indexed in GOogle Scholar - this work is funded by ESA for CHIME: The most common approach seems the use of DL over techniques such as thresholding (not considred ML) and ML/SVM for cloud detection (we have seen it with the papers above) used in works such as \cite{lebedeff2020board}. However, it's important to remember that the previous works, for instance from Phi-Sat-1 (high impact) is using CNN-based (so DL, not ML), and even also ref \cite{salazar2022cloud} pointed above to the fact that SVM is demonstrated (in RGB) to have lower performance compared to NU-net for cloud detection. JON: Also deep learning encodes a more complex knowledge in its structure and handles better the non-linear relationships and hence DL tends to be more accurate, and I would guess that the SVM could show a lower performance when it comes to distinguishing for instance clouds from snow/ice. Now referring to \cite{lebedeff2020board} next, the paper is for HSI image compression which is mandatory duento the large amount of data to transmit - remember high entropic sources (trend) + shannon channel depending on bandwidth and SNR (data bit rate) - clouds hide acquisition of interest. They apply selective compression across the spatial domain, i.e, they use LOWER BIT RATE ON CLOUDS (instead of the cloud screening referring to the cloud exclusion) AND HENCE A DEGRADATION IN CLOUDS WHILE PRESERVING THE REST WHICH IS NOT CLOUDS (BINARY CLASSIFICATION). The compression is based on CCSDS 123.0-B-2 [3 in \cite{lebedeff2020board}] with lossless or near-lossless compression (this relates again to the entropy and compression/loss of information). For this they use a prior cloud detection algorthm: they comapre the thresholding and ML/SVM. The threshold approach has been appløied to Lnadsat [4 in  ref \cite{lebedeff2020board}] and Sentinel-2 in ref [5 in  ref \cite{lebedeff2020board}]. Regarding SVM, in some cases they can be more demanding computationally than CNNs, especially for data such as HSI, according to ref [IEEE4201/Hardware Support Vector Machine (SVM) for satellite on-board applications]: "his paper proposes a hardware embedded SVM targeting space applications. The hardware SVM system allows the deployment of SVMs in various possible applications onboard spacecraft as it relieves the main processor from the computationally demanding calculations that are involved in SVM.", and then we can mention that the SVM has indeed been appied by Thales Alenia Space export program and other space missions according to ref \cite{lebedeff2020board} - here really give that reference. They also limit the dimension N of the feature space to the useful bands (they don't say how many bands, but okey the further confirm the need to reduce). The also insist on the FPR and the IMPORTANCE TO REDUCE THE FPR (JON: to reduce the loss of net data). 

%% \cite{gomez2006new}: this is just about how the problem of cloud detection (they mention they tried to increase the cloud detection accuracy) was being solved back in 2006 for Multispectral (JON: not HSI). Instead of airborne sensor, I like that they use the term space-brone sensors. Since this paper is from 2006 and mentions the spaceborne snesors working in the VNIR, we can see this is already coming since long time ago. Their approach has as steps: 1) Feature extraction, 2) Region of interest, 3) Image clustering and labeling, 4) Spectral unmixing <--- we would need to process this approach if needed (highlighted in the ref \cite{gomez2006new}). They actually address the problem of detecting the clouds over ice/snow. 

% \cite{pitonak2022cloudsatnet} - better understandable the \cite{giuffrida2020cloudscout} and better explained: mentions to CubeSats and I think it says they have less than 60 kg. Cost decrease of accessing the space. They present the CloudSatNet-1: an FPGA-based HW-accelerated quantized CNN for satellite on.board cloud coverage classificaiton - they explore the optiomal FPGA resource utilization. They mention there's a reduction in the memory footprint that allows the implementation in the low-cost FPGA Zynq-7020 from Xilinx (JON: HYPSO-1 was 7030 I think??). Again, the insist in the usage of only the RGB bands. They achieve 90% accuracy (when including image patches/tiles with snow and ice, then the performace is better to 94.4% - so snow and ice makes the performance drop a bit). NB: They use patches (it's obviously better for the memory footprint).  THE USE THREE BANDS: RED + GREEN + BLUE, in particular they use the following band codes (ref is to Sentinel-2): B2 (blue), B3 (green), B4 (red). MINMAX NORMALIZATION TO RE-SCALE THE DATA. They mention a false positive rate of 2.23% and that they use a 4-bit width model. They mention that with the maximum paralellization settings they achieved 2.5 W of average power consumption (0.2 W increase over the idle state) <-- I'm very unsure if this means that then the inference power consumption is 0.2 W (ask PGK if not clear? / seeing the reported power consumptions in the papers, I would be surprised if it was 0.2 W the consumption rather than 2.5 W, I really think 2.5 W makes more sense). Applies also to HSI. They mention the lightweight CNNs for cloud detection in comparison to previous SOA DNNs (the following DNNs are not so common I think): CDNetV1 [6 in ref \cite{pitonak2022cloudsatnet}], CDNetV2 [10 in \cite{pitonak2022cloudsatnet}] or CD-FM3SFs [33 in ref \cite{pitonak2022cloudsatnet}] - (confirm that these 3 last SOA networks are not lightweight). Refer to the Fig.7 in page 9/21 in ref \cite{pitonak2022cloudsatnet} with the CloudSatNet-1 Architecture and read the highlighted the details about the architecture on top (no bias, etc) - NB: they use the size 512x512x3 to compare against CloudScout Architecture in ref \cite{giuffrida2020cloudscout} - JON: It might be a good idea to crop for instance a HYPSO-1 image with 512x512 and compare the performance too, so repeat the same approach to compare against the CloudScout and also the CloudSatNet-1. Binary cross-entropy (binary classification): 0 (cloud level < 70%), 1 (cloud level > 70%). IMPORTANT: They have taken the binary cross-entropy formula and modified it to INCREASE THE PENALTY FOR FALSE POSITIVES refer to the formula (1) in page 9/21 in ref \cite{pitonak2022cloudsatnet}- NB: in Keras it seems you can indeed define your own method with the loss function. HYPER-PARAMETER TUNING: they follow the Bayesian optimnization aporoach and they give in table 2 page 11/21 the ranges for the parameters they change (NB: they don't change the number of filters, which is also an option, but the training parameters instead): learning rate, learning decay, batch size, and FP penalizer in the modified loss function. As evaluation metrics they use: accuracy, precision, recall, F1 score and FPR. IMPORTANT ABOUT QUANTIZATION (AGAIN SAME CONCLUSION): "we can concluse that the weights and activations quantization has a minimal or no effect on the model accuracy" and this is similar to the results achieved in \cite{salazar2022cloud} (our own conclusion from \cite{salazar2022cloud} as they didn't mention it directly) but it's something I observe. REGARDING BINARY CLASSIFICATION: They indeed mention that room for improivement is to provide multi-class isntead of binary classificcation, and although they don't say it explictly, this could be for instance the cloud composition or other multiclasses too e.g. [justo2023open]. 



%% \cite{giuffrida2020cloudscout}-THIS ARTICLE IS BNETTER EXPLAINED BUT I COULDN'T GO FULLY THROUGH IT YET (IT MIGHT BE REPETITION OF THE ABOVE) - FUNDED BY ESXA. They insist again in the 70% threshold to consider the images as fully cloudy or not. They insist again in the lack of data and on the emulation of the Hyperspecout-2 HS sensor due this lack of data. In the test set, they achieve 92% of accuracy, 1% of FPR, 1.8 W power consumption and 2.1 MB of emmory footprint (remember that in ref \cite{giuffrida2021varphi} it is mentioned a memmory footprint of kB rather than MB). Use terms: edge applications. In Section 3.1 in page 3/17 they have the overview of the ML accelerators: TPU [16 in ref \cite{giuffrida2020cloudscout}], GPU [18 in ref \cite{giuffrida2020cloudscout}], FPGA [19 in ref \cite{giuffrida2020cloudscout}], VPU [23 in ref \cite{giuffrida2020cloudscout}]. They point to a more extensive comparison among various COTS   for DL in [26, 27 in ref \cite{giuffrida2020cloudscout}]. They insist on using the best 3 BANDS THROUGH PCA. Refer to figure 7 for the CloudScat Network model - the network seems to be very compact. They point again to the modified categorical cross-entropy functuon. 


%% \cite{danielsen2021self}: Based on the conclusions section and SOA knowledge --> V: SOMS more interpretable than DNNs, faster to develop than DNNs (train, evaluate, and test), low complexity, trained from a few samples; X: SOMs are simple (not complex patterns), not use of spatial information and hence not accounting for spatial relationshoip / context and cannot handle then the possible misalignments as only spectral information is consdiered (misalignment is a common fact); unsupervised and its subsequent downs. 

%% \cite{langer2023robust} for application on HYPSO-1: insists on large volume of data and in the downlink bottlenbeck and mentions: "the key to overcoming the data badnwdith limitation  is to porocess the data on-board the satellite prior to downlink". The article presents an in-flight demonstration of the flexible on-board processing pipeline of the HYPSO-1 cube-sat with additional reliability and resiliencie analysis. FURTHER COMMENTS / IMPORTANT: Refer to highlighted in Conclusions page 18/23 and 19/23 - SVMs, decision trees, HYPSO-2 and HYPSO-3.


%% EXTRA REFS: 
%%  Sust. report: efforts to include AI for automation also in processing chain at the "marine level" ("sea surface level") and also from space (HYPSO-1, etc). 

% REGARDING HYPSO - DENNIS: 
% C code with input image and producing the segmented image or thumbnail if needed. An executable is produced
%   This executable is uploaded onboard and they only need to produce minor changes to interface the executable 
%   The process to produce the executable itself and the uploading to the satellite can just take around 2 days so it's 
%   fast. What takes more work is having the C code. JON: ARM Cortex (perhaps C implementation can also initially be     tested on the Zynq). JON: I think it would certainly be important to do a qualitative inspection of the generalization for other images to see how well the model generalizes, the qualitative analysis in unseen data is indeed also used in ref \cite{salazar2022cloud} where they use it for unseen data but even worse: from a different image sensor. The analysis should be with different exposure levels, times in the day, and scenes (this would be ideal) - and ofc, show also wrong results to see the room for improvement. JON: Consider if data augmentation could help the generalization of the model. NOTE: The image data is 6400x6400x3, but then the image patch (they use cropping) is 512x512x3 to match the input dimensions of the network to compare against the CloudScout network. 

%% EXTRA RESOURCES: 
% DevOps cycle
% For future integration on-board (C code + make executable + upload/Dennis): https://github.com/NTNU-SmallSat-Lab/onboard-pipeline-modules/tree/classification
% CRISP-DM methodology - often lack of understanding of the data and how to extract its value
% For previous paper, in OneDrive upload the wavelenghts which are the same for all and then this should be clarified in the README instructions document
% There should be a comparison with the baseline e.g.: for indian pines
% GANs (GenAI) for data augmentation (this only for training on-ground)
% In evaluation, the categorical class is computed from the largest probabily (this doesn't matter for the training which outputs a probgabily vector to train against a ground-truth one-hot encoded vector), so for checking the generalisation we will keep taking the largest probabily since this is what we have done for evaluation (the evaluation socres are calcuted over categorical annotations and predictions, not over probability vectors). However, we should bare in mind that it would of interest to try different thresholds. 
% Drawback of the ENVI tool
% BANDS TO USE - WHAT I SEE IN RECENT CAPTURES IS THAT THE FOLLOWING BANDS ARE USED: 18, 26, 67 (I should assume raw? - remember that in raw the wavelength is flipped, but I think it should refer to raw since HYPSO-1 downlinks raw, not radiance). 
% Another set-up for HYPSO for this year 2023 is 598x1092 instead of 956x684
% Distinguish: one thing is data point (a signature which is in 1D) and another thing is if we process it with 1D (only spectral context) or if we process it with 2D (spectral context + spatial context).
% How the dimensions change across the processing pipe, it's even more important in the 2D to not confuse the dimensions
% Mention that we have different modes: cropping, padding and how is this padding done and this is prior to patching
% Regarding patching: the step is set to PATCH_SIZE, so that means that the patches are not overlapping (non-overlapping patches). I ignore why sometimes overlapping patches are used.  
% I think that for the 2D case we would definitely need a pipeline block showing the subsequent processing - but this should be once it's clear and confirmed which processing steps we are following
% Data being the most valuable asset in the world, but similarity with oil in the sense that in raw there's no point. Possible: HYPSO Analytics Framework




% CONCLUSIONS RESEARCH QUESTIONS SENT EMAIL TAJ, RADU, LILY 13.09.2023:
        % Refers to the second article I’m starting to set the basis for. My intent now is to give you a short preliminary conclusion of the research questions that I am planning to formulate in the paper so that you can give me your feedback. The conclusion is based on a thorough study of the current state of the art. We will probably need around 3 pages just to describe the analysis as it has been quite extensive and it refers to a minimum of 30-40 articles connected to Cloud Detection in Satellite Imagery, including also relevant articles from ESA. NB: the context is neither purely Remote Sensing nor purely AI, but a combination of both. The context relates to the classification of clouds on-board HYPSO-1 using the HYPSO-1 Sea-Land-Clouds dataset and hence incorporating the additional classification of sea and land. In our shared document in Overleaf in the Introduction, I have plenty of notes (in comments) about the analysis I have made for 30 articles, but no need of course to go through them since they are just some draft notes I have taken. 
        
        
        % How does calibration influence classification performance?
        % At what stage in the on-board pipeline is calibration most effective?
        % How do SOA architectures, like those in Phi-1, perform on the HYPSO-1 dataset for cloud segmentation?
        % Which architecture should be selected comparing performance and complexity cost? Should HYPSO-1 aim at 1D or 2D CNN-based models (performance VS complexity trade-off)? 
        % How does the choice of hyperparameters impact the performance and robustness of cloud segmentation models on the HYPSO-1 dataset? 
        % How effectively do the models generalize to unlabeled ground truth data from HTYPSO-1?
        % Can we establish a benchmark of supervised learning models for inference on HYPSO-1? Would this serve to highlight the value of the HYPSO-1 dataset?
        % Is it feasible to design a system that simultaneously prioritizes the ranking of both clouds and water for HYPSO-1? In other words, how can we integrate cloud and water priority ranking systems into a unified decision-making framework for HYPSO-1 data users?
        % JON: NOT ADDED IN THE EMAIL: reducing the bands is obvious according to the state of the art, but we can check also how is the performance of the models before and after the reduction - does the performance degrade to much (the inference time should be smaller for reduced bands). It's important to highlight that these are metrics measured on PC. 
        
        % The preliminary questions above will be answered against the literature study I referred to above.
        % Experiments starting today (modifications to the current SW code are needed). The GPU is up and running to execute them. 


%% Feedback from Joe
%   Jon short comments: Joe also insists in the model simplicity, even if it's only one convolutional layer. 
        % Do something fast for on-board processing. We can have a model simple since the dataset is also simple when it comes to the number of classes it addresses, so then minimize the number of parameters being trained. We can keep a one-dimensional in CNN. But it would be recommendable to have a 2D U-Net and chop out some of the layers to make it simple. Then for the next paper we can focus on self-supervised and then more towards the end of the PhD (this is something I agree, I would complete first the process), we could explore doing clustering for 200 images for instance and then label instead of pixel by pixel, we could label the clusters (for that we would need to figure out what each cluster is). 
        % Joe asking if this network could be included (they give the network code): https://ieeexplore.ieee.org/document/9444141 - the code (also for the model architecture is on: https://github.com/danfenghong/IEEE_TNNLS_EGU-Net)
        % 

% WHAT: 
%  

\cite{salazar2022cloud}
\cite{spiller2022wildfire}
\cite{esposito2019orbit}
\cite{giuffrida2021varphi}
\cite{lebedeff2020board}
\cite{gomez2006new}
\cite{giuffrida2020cloudscout}
\cite{pitonak2022cloudsatnet}
\cite{danielsen2021self}
\cite{langer2023robust}
\cite{justo2022comparative}
\cite{justo2023open}
\cite{Article_AI_trends_citing_HYPSO1} % Refer to mission study
%%% MISSION STUDY - FURTHER LTERATURE



%%% TOMORROW: AND START BUILDING THE WHAT WITH REFERENCES (RESORTING WILL BE NEEDED THERE) (THEN WE WILL BE READY FOR THE HOW)





% \clearpage
% \vspace{-5pt} 
\section{Introduction}
\textcolor{blue}{Order to write: intro, method, results. Self-tip: WHAT + HOW.}

\lettrine[lines=2.5, lraise=0.1, nindent=0em]{T}{he} HYPSO-1 mission (...)



% WHAT - ARGUMENTATION TO ADDRESS (BUT IN GENERAL TERMS) - ADD EXTRA PT?: 
%   Context: General for solving sea/land/cloud classification in satellite platforms for Earth and ocean observation, and giving HYPSO-1 as an example. Why this is important and which source of novelty this has (any work for sea-land-clouds?). Contribution: inference activities in HYPSO-1 in the case example. Also same domain/context as in the same paper: marine environments (check the proportion of water) known for HAB events, etc. Benefits for platforms such as HYPSO when it comes to downlink times (reuse from previous draft from February) (analysis February). For different deep learning architectures, the performance and the viability for onboard processing (computational requirements). Novelty: configure-adjust the network with more than just increasing the kernel size and increasing the number of kernels, and conclude with the best architectures for HYPSO-1. For 20 extra images not included in the dataset, see how the model performs to see if it's realiable. Do we need quantified weights? (perhaps not for this paper; that can be a separate paper?)
%   1) How does radiance calibrate affect the classification performance? In other words, should classification be implemented prior or post calibration? 

% ZZZ: st. of the art - how to fit it

% SOA: 
%   Cloud detection onboard: CloudScout: A Deep Neural Network for On-Board Cloud Detection on Hyperspectral Images (MDPI) - prioritizing images onboard
%   Cloud Detection Autonomous System Based on Machine Learning and COTS Components On-Board Small Satellites - prioritizing images onboard (MDPI) - use of NU-Net for its regular use for cloud detection in RGB images - check Table 5 for Metric results of NU-Net and NU-Net-mod on the embedded device (I think they get lower than what we already get in the dataset paper). 
%  New cloud detection algorithm for multispectral and hyperspectral images: Application to ENVISAT/MERIS and PROBA/CHRIS sensors - I think they don't use ML/DL.
% IMPORTANT PAPER: In-orbit demonstration of artificial intelligence applied to hyperspectral and thermal sensing from space <-- I think it could have a bit of cloud detection, but still not sure at this point. <-- Refers to PhiSat-1 
% IMPORTANT PAPER: The Φ-Sat-1 Mission: The First On-Board Deep Neural Network Demonstrator for Satellite Earth Observation <-- Also mentions clod detection  <-- Refers to PhiSat-1 
% ON-BOARD CLOUD DETECTION AND SELECTIVE SPATIAL/SPECTRAL COMPRESSION BASED ON CCSDS 123.0-B-2 FOR HYPERSPECTRAL MISSIONS <-- I think this is mainly for compression for clouds (could be: adapting the CR?)
% Wildfire segmentation analysis from edge computing for on-board real-time alerts using hyperspectral imagery <-- It's for wildfire detection from satellites, but it also mentions phi-1, and it's also a detection applic.
% CloudSatNet-1: FPGA-Based Hardware-Accelerated Quantized CNN for Satellite On-Board Cloud Coverage Classification <-- FPGA implementation but for cloud detection, considers also the effects of the quantization
% Self-Organizing Maps for Clustering Hyperspectral Images On-Board a CubeSat <- Aksel, TAJ; mention to water, land and clouds (HYPSO-1 dataset addresses this). 
% Robust and Reconfigurable On-Board Processing for a Hyperspectral Imaging Small Satellite <-- Dennis paper some mentions


%   



% EXPERIMENTS: 
%   Same network as in the paper - raw vs calibrated 
%   1D Networks:
%       LucasResNet
%       LucasCoordConv
%   NB!!! Use of lightweight DLNN is key (for sema. segmentation), for instance: MobileNet - check other examples

%   2D Networks (for now: process entire image, so no patching): 
%       U-Net
%       Reduced UNet (Simen N.) - I see unet_model, quantized_unet_model, cloud_masking_unet

%       C-UNet++ (Sondre) - cunet, cunet_adapted, cunet_plus, cunet_plus_adapted, cunet_plus_adapted_dropout. For quantified: q_cunet_plus, test_net, build_qunet_plus, build_qunet_plus_adapted, q_cunet_plus_adapted

%   Patching here 
%       MD-Unet
%       Mask RCNN based on the Fast-RCNN
%   NB: Consider the attention mechanisms afterwards
%   NB: Consider also ensemble / multi-model approach through majority voting (for this the models would need to be extremely simple for onboard processing). 

%   NB: Do hyper-parameter tuning optimization now that we have the GPU


%% ZZZ check the compact versions from Simen/Sondre (find the thesis)
%% ZZZ Target application conference - first week of October - TAJ, Radu, Lily. GPU notif. 
%% ZZZ Cotribution Lily: SoA


% ZZZ Consult with Marie research question 1) since for overexposed we will be in principle calibrating it anyway (actually we've done so in the paper), but we can still try to the classification I think. 



% Pipeline: training over raw or over calobrated? Any difference? 
% How different models perform on the dataset: any specific with higher performance? Viability for onboard
% How would attention blocm work? 
% JON--- IMPORTANT revise 03 or 04/09/23 HSI Deep Learning Classification
%%      Attention in Liuetal 
%%      2D U-Net
%%      Attention in 2D U-Net
%%      CUNet and attention in CUNet
%%%     Mask RCNN to classifiy at pixel level
%%%     MD-UNet with attention



%% Sorting issue in the overexposed spectra in web dataset paper



%%% The comments below are from the dataset paper
 % JON / Commented out the part for the different sensors: We provide an overview of well-known HSI datasets in the state of the art. Namely, Indian Pines, Salinas, Cuprite, Houston, Jasper Ridge, Urban, and Kennedy Space Centre, acquired from the airborne AVIRIS sensor. Additionally, datasets from the airborne ROSIS sensor, such as Pavia Centre and Pavia University, and the Washington DC Mall dataset from the HYDICE sensor, along with the SAMSON dataset. 
 % JON / Commented out for next paper: the datasets (not the Kennedy Space Center and the Jasper Ridge, but the ones that we mention in tihis paper) include basically land cover types and I have removed the examples: including urban areas, mining regions, and agricultural regions with crops, grass, woods, buildings, and structures.
 % JON / comment out the part about unsupervised learning: %In contrast, unsupervised learning uncovers hidden patterns from unlabeled data, reducing manual labeling and potential model bias. However, interpreting predictions from unsupervised models may be ambiguous without labeled guidance. Therefore, despite time-consuming data labeling, supervised learning remains widely accepted for explainable predictions. 

% JON - Of interest about Hyperspectral Imaging (provided by TAJ email): Filling the gap: Hyperspectral lessons from the great wet barnyard of Long Island Sound - Heidi M. Dierssen, University of Connecticut: 
    % Satellites provide unprecedented views of the swirling, dynamic patterns of ocean life. Even though we cannot directly see the microscopic phytoplankton that fuel the ocean food web from space, we can see how they absorb and scatter light as they photosynthesize. The evolution of chlorophyll-a derived from satellites over the last twenty years has outlined fronts where fish congregate, intense algal blooms that can be toxic, and changes in productivity of the vast deserts in the center of ocean gyres. Sensor technology has improved considerably over the last few decades and space-borne sensors that provided only 3 to 8 channels of information in visible wavelengths are now “hyperspectral” with 100’s of channels across the same visible spectrum of light.  New missions like NASA’s upcoming Plankton Aerosol Cloud and ocean Ecosystem (PACE) mission will better quantify how the ocean and atmosphere breathe through exchange of carbon dioxide and oxygen – the “lungs” of the planet. What makes the hyperspectral sensor unique is that it can provide a spectral “fingerprint” for monitoring the biodiversity of photosynthesizing flora and fauna in the water column, on the seafloor, and floating on the sea surface. Here, I will draw from optical research conducted in my lab over the last decade in Long Island Sound (LIS), the largest urban estuary in the U.S. with 9 million people living within the watershed.  Highly impacted by human activities, F. Scott Fitzgerald (1925) referred to LIS as “the most domesticated body of salt water in the Western hemisphere, the great wet barnyard of Long Island Sound.” Field data from this dynamic and optically complex estuary illustrate how multi-spectral imagery is not sufficient to characterize phytoplankton dynamics and how hyperspectral measurements will allow us to better quantify phytoplankton changes through time.
     






